Crossing Rays: Evaluation of Bimanual Mid-air Selection Techniques in an Immersive Environment

Mid-air navigation offers a method of aerial travel that mitigates the constraints associated with continuous navigation. A mid-air selection technique is essential to enable such navigation. In this paper, we consider four variations of intersection-based bimanual mid-air selection techniques with visual aids and supporting features: Simple-Ray, Simple-Stripe, Precision-Stripe, and Cursor-Sync. We evaluate their performance and user experience compared to an unimanual mid-air selection technique using two tasks that require selecting a mid-air position with or without a reference object. Our findings indicate that the bimanual techniques generally demonstrate faster selection times compared to the unimanual technique. With a supporting feature, the bimanual techniques can provide a more accurate selection than the unimanual technique. Based on our results, we discuss the effect of selection technique's visual aids and supporting features on performance and user experience for mid-air selection.

==> ANOVA_Result_contents/4_result.tex <==
\section{Result}

This section reports the results of our user study. We utilized a two-way repeated measures Analysis of Variance (ANOVA) test, with a significance level of 5\%, to analyze selection time, error distance, and user experience responses (measured by NASA-TLX and UEQ) for each task. Additionally, we applied the Geisser-Greenhouse correction to guard against potential violations of the sphericity assumption.
The post-hoc test is conducted by Fisher's least significant differences (LSD) pairwise comparison with $\alpha$ = .05 level for significance. We employ the median as the representative value for our analysis to mitigate the potential skewness of the collected data.

\subsection{Task 1 Results}
\subsubsection{Selection Time}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{figures/selection_time_withB.pdf}
\caption{
Task 1 - Selection Time: Selection time result for each technique and distance (95\% CI error bar). 
} 
\label{figure:RT_W/R}   
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{figures/error_distance_withB.pdf}
\caption{
Task 1 - Error Distance: The error distance between the selected position distance from the target position for each technique and distance conditions (95\% CI error bar).
} 
\label{figure:ED_W/R}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/button_clicks_with_box.pdf}
\caption{
Task 1 - Button Clicks: The number of button clicks for each technique and distance (95\% CI error bar). 
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:AT_W/R}   
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/TLX_with_box.pdf}
\caption{
Task 1 - NASA-TLX result: Questionnaire result for each subsection (95\% CI error bar).
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:TLX_W/R}   
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/UEQ_with_box.pdf}
\caption{
Task 1 - UEQ result: Questionnaire result for each subsection (95\% CI error bar).
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:UEQ_W/R}   
\end{figure}

The ANOVA results of selection time are reported in Figure \ref{figure:RT_W/R}. % and Table \ref{table:RT_W/R}.
There is an interaction effect between the technique and distance (F(8, 152) = 7.247, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .276).
% Interaction: each technique condition
% \ic{simple effects at 3m, 6m, 9m}
%\ic{add all conditions} have the fastest target position selection at 3m (Simple: M = 2.751s, SD = 1.245; Simple-Stripe: M = 2.543s, SD = 0.893; Precision-Strip: M = 3.692s, SD = 1.448;  and Cursor-Sync: M = 3.843s, SD = 1.561), at 6m is the next (Simple: M = 3.760s, SD = 1.241, $p$ \textless .001; Simple-Stripe: M = 3.603s, SD = 1.110, $p$ \textless .001; Precision-Strip: M = 5.039s, SD = 2.036, $p$ \textless .001;  and Cursor-Sync: M = 4.323s, SD = 1.510, $p$ \textless .001), and at 9m is the slowest (Simple: M = 5.688s, SD = 2.161,  $p$ \textless .001; Simple-Stripe: M = 6.034s, SD = 2.232, $p$ \textless .001; Precision-Strip: M = 6.866s, SD = 2.734, $p$ \textless .001;  and Cursor-Sync: M = 5.968s, SD = 1.758, $p$ \textless .001). \ic{explain it as simple effects by meters,e.g., at 3m what's faster? }
%However, the One-Hand Simultaneous technique selection at 3m (M = 5.728s, SD = 2.599) is not significantly different from that under 6m and 9m conditions.
%But the 6m target positions' result (M = 5.325s, SD = 2.399, $p$ \textless .001) is significantly faster than the result at 9m (M = 6.542s, SD = 2.700), like a bimanual technique's result.
% Interaction: each distance condition
Further analysis reveals that there are simple effects on technique at 3m (F(1.807, 34.336) = 24.627, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .564) and 6m (F(2.626, 49.890) = 10.394, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .354). However, there is no simple effect at 9m ($p$ = .164). % (F(4,76) = 1.678, $p$ = .164, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .081).
Pairwise comparisons reveal that, at the 3m target position, Simple-Ray has faster selection time (M = 2.75s, SD = 1.25) than Precision-Stripe (M = 3.69s, SD = 1.45, $p$ \textless .001), Cursor-Sync (M = 3.84s, SD = 1.56, $p$ = .002), and One-Hand Simultaneous (M = 5.73s, SD = 2.6, $p$ \textless .001).
% simple = Simple-Stripe > others
In addition, Simple-Stripe leads to faster selection time (M = 2.54s, SD = 0.89) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ = .002), and One-Hand Simultaneous ($p$ \textless .001). Furthermore, One-Hand Simultaneous has a significantly faster than Precision-Stripe ($p$ = .002) and Cursor-Sync ($p$ \textless .001).

At 6m, Simple-Ray has a faster selection time (M = 3.76s, SD = 1.24) than Precision-Stripe (M = 5.04s, SD = 2.04, $p$ = .002) and One-Hand Simultaneous (M = 5.33s, SD = 2.40, $p$ \textless .001).
Simple-Stripe also has a faster selection time (M = 3.60s, SD = 1.11) than Precision-Stripe ($p$ \textless .001), Cursor-Sync (M = 4.32s, SD = 1.51, $p$ = .027), and One-Hand Simultaneous ($p$ \textless .001).
Moreover, Cursor-Sync has a faster completion time than the Precision-Stripe ($p$ = .033) and One-Hand Simultaneous ($p$ = .008).

There is a main effects on technique (F(4, 76) = 10.480, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .36).
Pairwise comparisons show that Simple-Ray (M = 4.07s, SD = 2.00) has a faster selection time than Precision-Stripe (M = 5.20s, SD = 2.48, $p$ = .004), Cursor-Sync (M = 4.71s, SD = 1.83, $p$ = .042), and One-Hand Simultaneous (M = 5.87s, SD = 2.58, $p$ \textless .001).
In addition, Simple-Stripe also results (M = 4.06s, SD = 2.11) faster than Precision-Stripe ($p$ = .009), Cursor-Sync ($p$ = .044), and One-Hand Simultaneous ($p$ \textless .001).
Moreover, Cursor-Sync is significantly faster than One-Hand Simultaneous ($p$ \textless .001).

A significant main effect is found on distance (F(1.552, 29.496) = 114.720, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .86).
Pairwise comparisons reveal that 3m (M = 3.71s, SD = 1.98) has a faster selection time than 6m (M = 4.41s, SD = 1.83, $p$ \textless .001) and 9m (M = 6.22s, SD = 2.34, $p$ \textless .001).
In addition, 6m is faster than 9m ($p$ \textless .001).
These results partially support \textbf{H1} and \textbf{H2}.

\subsubsection{Error Distance}

The results are reported in Figure \ref{figure:ED_W/R}.
A significant main effect is found on technique (F(4, 76) = 8.251, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .303).
Pairwise comparisons show that Simple-Ray has a smaller error distance (M = 22.26cm, SD = 6.77) than Simple-Stripe (M = 26.6cm, SD = 8.21, $p$ \textless .001), Cursor-Sync (M = 26.86cm, SD = 9.86, $p$ = .005), and One-Hand Simultaneous (M = 27.91cm, SD = 8.64, $p$ = .003).
In addition, Precision-Stripe has a significantly lower error distance (M = 20.35cm, SD = 7.32) than Simple-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ = .002).
These results do not support H3 and H4.

\subsubsection{Button Clicks}
The results of the number of button clicks are reported in Figure \ref{figure:AT_W/R}. % and Table [].
There is an interaction effect between technique and  distance (F(3.476, 66.041) = 16.239, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .461).
Further analysis reveals that there are simple effects on technique at 6m (F(1.836, 34.879) = 4.563, $p$ = .020, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = 194) and 9m (F(2.465,46.831) = 23.826, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .556).
Pairwise comparisons reveal that, at the 6m target position, Simple-Ray has more button clicks (M = 1.60, SD = 1.00) than Cursor-Sync (M = 1.03, SD = 0.11, $p$ = .012) and One-Hand Simultaneous (M = 1.03, SD = 0.11, $p$ = .020).
In addition, Simple-Stripe leads to more button clicks (M = 1.50, SD = 0.63) than Cursor-Sync ($p$ = .001) and One-Hand Simultaneous ($p$ = .004).

At 9m, Simple-Ray has more button clicks (M = 2.65, SD = 1.26) than Precision-Stripe (M = 1.58, SD = 0.82, $p$ = .002), Cursor-Sync (M = 1.08, SD = 0.34, $p$ < .001), and One-Hand Simultaneous (M = 1.00, SD = 0.00, $p$ < .001).
In addition, Simple-Stripe (M = 3.10, SD = 1.35) has more button clicks than Precision-Stripe ($p$ = .002), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).

There are main effects on technique (F(2.111, 40.113) = 18.430, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .492) and distance (F(1.403, 26.658) = 67.413, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .780).
Pairwise comparisons show that Simple-Ray has more button clicks (M = 1.79, SD = 1.13) than Precision-Stripe (M = 1.28, SD = 0.60, $p$ = .011), Cursor-Sync (M = 1.05, SD = 0.24, $p$ \textless .001), and One-Hand Simultaneous (M = 1.04, SD = 0.21, $p$ \textless .001).
In addition, Simple-Stripe (M = 1.89, SD = 1.23) has more button clicks than Precision-Stripe ($p$ = .002), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).
Furthermore, Precision-Stripe has more attempts than Cursor-Sync ($p$ = .029) and One-Hand Simultaneous ($p$ = .008).

Pairwise comparisons show that 3m (M = 1.08, SD = 0.27) has more button clicks than 6m (M = 1.28, SD = 0.62, $p$ \textless .001) and 9m (M = 1.88. SD = 1.24, $p$ < .001). In addition, 6m has more button clicks than 9m ($p$ \textless .001).

\subsubsection{NASA-TLX}

The results of the NASA-TLX are presented in Figure \ref{figure:TLX_W/R}. 
\paragraph{Effort}
There is a main on Effort (F(4, 76) = 3.244, $p$ = .016, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .146).
A pairwise comparison shows that Precision-Stripe (M = 2.80, SD = 1.67)  has a lower effort rate than Simple-Stripe (M = 3.55, SD = 1.79, $p$ = .014) and One-Hand Simultaneous (M = 3.75, SD = 1.71, $p$ = .016).
In addition, Cursor-Sync (M = 2.70, SD = 1.81) has a lower Effort rate than Simple-Stripe ($p$ = .034) and One-Hand Simultaneous ($p$ = .018).

\paragraph{Frustration}
There is also a main effect on Frustration (F(2.556, 48.745) = 5.293, $p$ = .005, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .218).
Pairwise comparisons reveal that Precision-Stripe has a lower Frustration rate (M = 1.65, SD = 1.14) than Simple-Ray (M = 2.85, SD = 2.03, $p$ = .006), Simple-Stripe (M = 2.80, SD = 1.82, $p$ = .003), Cursor-Sync (M = 1.90, SD = 1.48, $p$ = .016), and One-Hand Simultaneous (M = 2.60, SD = 1.93, $p$ = .040).
In addition, Cursor-Sync has a lower Frustration rate than Simple-Ray ($p$ = .040).

There are no significant main effects on Mental Demand, Physical Demand, Performance, and Temporal Demand on technique.

\subsubsection{UEQ}
The results of the UEQ are presented in Figure \ref{figure:UEQ_W/R}. 
\paragraph{Attractiveness}
There is a main effect on Attractiveness (F(2.109, 40.065) = 3.338, $p$ = .043, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .149).
Pairwise comparisons show that Cursor-Sync has a higher Attractiveness rate (M = 1.42, SD = 1.22) than Simple-Ray (M = 0.63, SD = 1.23, $p$ = .021) and Simple-Stripe (M = 0.90, SD = 1.24, $p$ = .047).

\paragraph{Efficiency}
There is a main effect on Efficiency (F(4, 76) = 3.381, $p$ = .013, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .151).
Cursor-Sync has higher Efficiency rate (M = 1.74, SD = 0.87) than Simple-Stripe (M = 1.05, SD = 1.21, $p$ = .037) and One-Hand Simultaneous (M = 0.85, SD = 1.27, $p$ = .020).
In addition, Precision-Stripe has a higher Efficiency rate (M = 1.60, SD = 0.84) than One-Hand Simultaneous (M = 0.85, SD = 1.27, $p$ = .036).

\paragraph{Dependability}
There is a main effect on Dependability (F(4, 76) = 4.712, $p$ = .002, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .199). 
Comparisons show that Precision-Stripe has a higher Dependability rate (M = 1.29, SD = 0.87) than Simple-Ray (M = 0.74, SD = 1.02, $p$ = .036) and One-Hand Simultaneous (M = 0.78, SD = 0.97, $p$ = .023).
In addition, Cursor-Sync (M = 1.50, SD = 1.01) has higher Dependability rate than Simple-Ray (M = 0.74, SD = 1.02, $p$ = .005), Simple-Stirpe (M = 0.98, SD = 1.19, $p$ = .032), and One-Hand Simultaneous (M = 0.78, SD = 0.97, $p$ = .006).

There is no significant difference in Novelty, Perspicuity, and Stimulation among techniques.

\subsection{Task 2 Results}
\subsubsection{Selection Time}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/response_time_without_box.pdf}
\caption{
Task 2 - Selection Time result: Selection time results for each technique and distance (95\% CI error bar).
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:RT_O/R}   
\end{figure}

The selection time results in task 2 with each condition are reported in Figure \ref{figure:RT_O/R}.
These results show an \textbf{interaction effect} between the technique type and the target position distance (F(8, 152) = 13.324, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .412).
Further analysis reveals that there are simple effects on technique at 3m (F(1.944, 36.929) = 72.526, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .792), 6m (F(4, 76) = 49.594, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .723), and 9m (F(4, 76) = 59.515, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .758).
Pairwise comparisons reveal that, at the 3m target position, Simple-Ray has faster selection time (M = 1.71s, SD = 0.73) than Precision-Stripe (M = 2.90s, SD = 0.77, $p$ \textless .001), Cursor-Sync (M = 2.52s, SD = 0.73, $p$ \textless .001), and One-Hand Simultaneous (M = 5.05s, SD = 1.46, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 1.88s, SD = 0.60) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).
Furthermore, Precision-Stripe has a significantly faster selection than One-Hand Simultaneous ($p$ \textless .001).
Lastly, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .037) and One-Hand Simultaneous ($p$ \textless .001).

At 6m, Simple-Ray has faster selection time (M = 2.13s, SD = 1.06) than Precision-Stripe (M = 4.19s, SD = 1.39, $p$ \textless .001), Cursor-Sync (M = 3.47s, SD = 1.06, $p$ \textless .001), and One-Hand Simultaneous (M = 4.67s, SD = 1.39, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 2.35s, SD = 0.63) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).
Furthermore, Precision-Stripe has a significantly faster selection than One-Hand Simultaneous ($p$ = .037).
Lastly, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .014) and One-Hand Simultaneous ($p$ \textless .001).

At 9m, Simple-Ray has faster selection time (M = 2.41s, SD = 1.22) than Precision-Stripe (M = 5.22s, SD = 1.92, $p$ \textless .001), Cursor-Sync (M = 4.39s, SD = 1.37, $p$ \textless .001), and One-Hand Simultaneous (M = 5.44s, SD = 1.45, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 2.60s, SD = 0.71) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).
Furthermore, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .011) and One-Hand Simultaneous ($p$ \textless .001).

There are main effects on technique (F(4, 76) = 88.065, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .823) and distance (F(2, 38) = 56.226, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .747).

Pairwise comparisons show that Simple-Ray (M = 2.08s, SD = 1.05) has a faster selection time than Precision-Stripe (M = 4.11s, SD = 1.71, $p$ \textless .001), Cursor-Sync (M = 3.46s, SD = 1.31, $p$ \textless .001), and One-Hand Simultaneous (M = 5.05s, SD = 1.45, $p$ \textless .001).
In addition, Simple-Stripe has a faster result (M = 2.28s, SD = 0.71) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001)
Furthermore, Simple-Stripe has a faster completion time than One-Hand Simultaneous ($p$ \textless .001), and Cursor-Sync has a faster completion time than Precision-Stripe ($p$ = .008) and One-Hand Simultaneous ($p$ \textless .001).

Pairwise comparisons show that 3m (M = 2.81s, SD = 1.50) is faster than 6m (M = 3.36s, SD = 1.50, $p$ \textless .001) and 9m (M = 4.01s, SD = 1.87, $p$ \textless .001).
In addition, 6m is faster than  9m ($p$ \textless .001).
These results support \textbf{H1} and \textbf{H2}.

\subsubsection{Error Distance}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/error_distance_without_box.pdf}
\caption{
Task 2 - Error Distance: The error distance between the selected position distance from the target position for each technique and distance conditions (95\% CI error bar).
} 
\label{figure:ED_O/R}   
\end{figure}

The error distance results with each condition are reported in Figure \ref{figure:ED_O/R}.
There is an interaction effect between technique and target position distance (F(8, 152) = 11.634, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .380).
Further examination shows significant simple effects of the techniques at distances of 3m (F(2.505, 47.596) = 24.371, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .562), 6m (F(4, 76) = 12.079, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .389), and 7m (F(1.755, 33.350) = 9.300, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .329).

Pairwise comparisons show that, with a 3m located target, One-Hand Simultaneous (M = 50.60cm, SD = 21.37, $p$ \textless .001) has significantly lower accurate rates than Simple-Ray (M = 22.50cm, SD = 14.30), Simple-Stripe (M = 17.61cm, SD = 9.25),  Precision-Stripe (M = 18.80cm, SD = 14.69) and Cursor-Sync (M = 14.83cm, SD = 7.37).
In addition, Simple-Ray is less accurate than the Cursor-Sync ($p$ = .041) technique.

With a 6m condition,  Simple-Stripe has more accurate results (M = 51.68cm, SD = 23.42) than Simple-Ray (M = 70.58cm, SD = 40.13, $p$ = .025) and One-Hand Simultaneous (M = 91.70cm, SD = 49.75, $p$ = .001).
Precision-Stripe is also more accurate (M = 42.04cm, SD = 34.58) than Simple-Ray ($p$ = .002) and One-Hand Simultaneous ($p$ \textless .001). 
Moreover, Cursor-Sync is more accurate (M = 32.72cm, SD = 19.74) than Simple-Ray ($p$ \textless .001), Simple-Stripe ($p$ = .014), and One-Hand Simultaneous ($p$ \textless .001) techniques.

With a 9m condition, Simple-Ray is less accurate (M = 161.01cm, SD = 117.66) than Precision-Stripe (M = 77.78cm, SD = 32.08, $p$ = .002), Cursor-Sync (M = 66.33cm, SD = 35.23, $p$ \textless .001), and One-Hand Simultaneous (M = 71.42cm, SD = 32.26, $p$ = .006).
Simple-Stripe technique is also less accurate (M = 114.71cm, SD = 45.74) than Precision-Stripe ($p$ = .013), Cursor-Sync ($p$ = .003), and One-Hand Simultaneous ($p$ = .001).

There are main effects on technique (F(4, 76) = 9.294, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .328) and distance (F(2, 38) = 90.853, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .827). 
Pairwise comparisons show that Precision-Stripe has a less error distance (M = 46.21cm, SD = 37.21) than Simple-Ray (M = 84.70cm, SD = 91.63, $p$ \textless .001) and One-Hand Simultaneous (M = 71.24cm, SD = 39.57, $p$ = .002).
In addition, Cursor-Sync has a less error distance (M = 37.96cm, SD = 31.72) than Simple-Ray ($p$ \textless .001), Simple-Stripe (M = 61.34cm, SD = 50.23, $p$ = .004), Precision-Stripe ($p$ = .046), and One-Hand Simultaneous ($p$ \textless .001).
Lastly, the participants complete the task more accurately when a target position is 3m (M = 24.87cm, SD = 19.20) than 6m (M = 57.74cm, SD = 40.54, $p$ \textless .001) and 9m (M = 98.25cm, SD = 70.57, $p$ \textless .001), and also, the result from 6m is more accurate than from 9m ($p$ \textless .001).

\subsubsection{NASA-TLX}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/TLX_without_box.pdf}
\caption{
Task 2 - NASA-TLX result: Questionnaire result for each subsection (95\% CI error bar).
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:TLX_O/R}   
\end{figure}

The NASA-TLX results are shown in Figure \ref{figure:TLX_O/R}.

\paragraph{Mental Demand}
There is a main effect on Mental Demand (F(3.071, 58.341) = 4.572, $p$ = .006, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .194).
Pairwise comparisons show that One-Hand Simultaneous has a higher Mental Demand rate (M = 4.25, SD = 1.94) than Simple-Ray (M = 3.15, SD = 1.66, $p$ = .005), Simple-Stripe (M = 2.85, SD = 1.79, $p$ = .001), Precision-Stripe (M = 3.00, SD=1.69, $p$ = .008), and Cursor-Sync (M = 3.10, SD = 1.97, $p$ = .012).

\paragraph{Performance}
 In addition, there is a significant main effect on Performance (F(4, 76) = 7.458, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .282).
 One-Hand Simultaneous has (M = 3.65, SD = 1.50) lower performance rate than Simple-Ray (M = 4.85, SD = 1.76, $p$ \textless .001), Simple-Stripe (M = 4.95, SD = 1.61, $p$ \textless .001), Precision-Stripe (M = 5.35, SD = 1.57, $p$ \textless .001), and Cursor-Sync (M = 4.80, SD = 1.61, $p$ \textless .001).

\paragraph{Effort}
There is a main effect on Effort (F(4, 76) = 5.153, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .213).
One-Hand Simultaneous has higher Effort rate (M = 4.00, SD = 1.89) than Simple-Ray (M = 3.25, SD = 1.89, $p$ = .021), Simple-Stripe (M = 2.80, SD = 1.40, $p$ = .006), and Cursor-Sync (M = 2.75, SD = 1.68, $p$ = .002).
However, there is no difference between One-Hand Simultaneous and Precision-Stripe, and among Simple-Ray, Simple-Stripe, and Cursor-Sync.

There is no significant main effect on Frustration, Physical Demand, and Temporal Demand. 

\subsubsection{UEQ}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/UEQ_without_box.pdf}
\caption{
Task 2 - UEQ result: Questionnaire result for each subsection (95\% CI error bar).
} 
\label{figure:UEQ_O/R}   
\end{figure}

The results of UEQ are presented in Figure \ref{figure:UEQ_O/R}.

\paragraph{Attractiveness}
There is a main effect on Attractiveness (F(2.385, 45.323) = 8.370, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .306).
Pairwise comparisons show that One-Hand Simultaneous has a lower Attractiveness rate (M = 0.18, SD = 1.57) than Simple-Ray (M = 1.18, SD = 1.11, $p$ \textless .001), Simple-Stripe (M = 1.14, SD = 1.51, $p$ = .012), Precision-Stripe (M = 1.58, SD = 1.12, $p$ \textless .001), and Cursor-Sync (M = 1.31, SD = 1.16, $p$ = .003 ).
In addition, Simple-Stripe has a lower Attractiveness rate than Precision-Stripe ($p$ = .022).

\paragraph{Efficiency}
There is a main effect on Efficiency (F(2.304, 43.789) = 5.422, $p$ = .006, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .222).
One-Hand Simultaneous has a lower Efficiency rate (M = 0.79, SD = 1.24) than Simple-Ray (M = 1.59, SD = 0.80, $p$ = .011), Simple-Stripe (M = 1.58, SD = 1.11, $p$ = .039), Precision-Stripe (M = 1.75, SD = 0.86, $p$ = .005), and Cursor-Sync (M = 1.81, SD = 0.97, $p$ = .008).

\paragraph{Dependability}
Moreover, there is a main effect on Dependability (F(2.220, 42.171) = 6.887, $p$ = .002, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .266).
One-Hand Simultaneous  has a lower Dependability rate (M = 0.37, SD = 1.21) than Simple-Ray (M = 1.09, SD = 0.94, $p$ = .029), Simple-Stripe (M = 1.24, SD = 0.88, $p$ = .005), Precision-Stripe (M = 1.39, SD = 0.84, $p$ = .002), and Cursor-Sync (M = 1.33, SD = 0.97, $p$ = .006). 

\paragraph{Perspicuity}
There is a main effect on Perspicuity (F(2.486, 47.228) = 6.418, $p$ = .002, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .253).
One-Hand Simultaneous has a lower perspicuity rate (M = 1.10, SD = 1.32) than Simple-Ray (M = 2.31, SD = 0.81, $p$ \textless .001),  Simple-Stripe (M = 2.04, SD = 1.28, $p$ = .007), Precision-Stripe (M = 2.11, SD = 1.02, $p$ = .002), and Cursor-Sync (M = 2.00, SD = 1.23, $p$ = .026).

\paragraph{Stimulation}
Lastly, there is a main effect on Stimulation (F(4, 76) = 4.260, $p$ = .004, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .183).
One-Hand Simultaneous (M = 0.23, SD = 1.34) has a lower Stimulation rate than Simple-Ray (M = 0.86, SD = 1.23, $p$ = .020), Precision-Stripe (M = 1.21, SD = 1.19, $p$ = .011) and Cursor-Sync (M = 1.20, SD = 0.97, $p$ = .006).
However, there is no significant difference between One-Hand Simultaneous and Simple-Stripe (M = 0.88, SD = 1.48).

The Novelty of each technique is not significantly different in this task.

==> ANOVA_Result_contents/4_result_large_table.tex <==
\section{Results}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/selection_time_with_box.pdf}
% {ANOVA_Result_contents/figures/response_time_with_box.pdf}
\caption{
Task 1 - Selection Time results with 95\% CI:
\dhk{
Lower values indicate better/faster performance, whereas higher values signify poorer performance.
% Higher indicates worse performance (delayed) and lower indicates better performance (quick).
}
} 
\label{figure:RT_W/R}   
\end{figure}



This section reports the study results.
We utilized a two-way repeated measures Analysis of Variance (ANOVA) test, with a significance level of 5\%, to analyze selection time, error distance, and user experience responses (measured by NASA-TLX and UEQ) for each task. Additionally, we applied the Geisser-Greenhouse correction to guard against potential violations of the sphericity assumption.
The post-hoc test is conducted by Fisher's least significant differences (LSD) pairwise comparison with $\alpha$ = .05 level for significance.
We employ the median as the representative value for our analysis to mitigate the potential skewness of the collected data.

% \subsection{Task 1 Results}
\subsection{Results: Task 1 \dhk{- \textit{with Reference}}}

\subsubsection{Selection Time}


\begin{table}
\centering
% \caption{With-Reference task: selection time results with the technique and distance conditions}
\caption{Task 1 - Selection Time results with ANOVA analysis. There are interaction effects at 3m and 6m and main effects on technique and distance. M: Mean selection time (s), SD: Standard Deviation, $p_{_{XX}}$: p-value for a comparison with XX, ns: not significant, $*$: $p$ \textless .05, $**$: $p$ \textless .01, $***$: $p$ \textless .001}
% \begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.5cm}| m{0.5cm} | m{1.6cm} | m{1.9cm}| m{2.2cm} | m{1.8cm}| m{1.5cm}}
\begin{tabular} {m{1.43cm} | m{0.7cm} | m{0.54cm} | m{0.457cm} | m{0.457cm}| m{0.457cm}| m{0.457cm}| m{0.457cm}}
\toprule 
\multicolumn{8}{c}{\textbf{Interaction effect}} \\ \midrule
    {\textbf{}} & \multicolumn{3}{c|}{\textbf{F}} & \multicolumn{2}{c|}{\textbf{$p$}} & \multicolumn{2}{c}{\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
    \multicolumn{1}{l|}{{Interaction}} & \multicolumn{3}{c|}{F(8, 152) = 7.25}    &   \multicolumn{2}{c|}{***}    &   \multicolumn{2}{c}{.276}\\ \midrule \midrule
    \multirow{2}{*}{\hspace{0.5cm}\vspace{-0.15cm}3m} & \multicolumn{3}{c|}{F(1.8, 34.3) = 24.6} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.564}\\ \cmidrule{2-8}
         & \multicolumn{1}{c|}{M} & \multicolumn{1}{c|}{SD} & \multicolumn{1}{c|}{$p_{_{SR}}$}& \multicolumn{1}{c|}{$p_{_{SS}}$}& \multicolumn{1}{c|}{$p_{_{PS}}$}& \multicolumn{1}{c|}{$p_{_{CS}}$}& \multicolumn{1}{c}{$p_{_{OH}}$}\\ \midrule
        \multicolumn{1}{c|}{SR} & \multicolumn{1}{c|}{2.75} & \multicolumn{1}{c|}{1.25} & {-} & {ns}& {***} & {**} & {***}\\
        \multicolumn{1}{c|}{SS} & \multicolumn{1}{c|}{2.54} & \multicolumn{1}{c|}{0.89} & {-} & {-} & {***} & {**} & {***}\\
        \multicolumn{1}{c|}{PS} & \multicolumn{1}{c|}{3.69} & \multicolumn{1}{c|}{1.45} & {-} & {-} & {-} & {ns} & {**}\\
        \multicolumn{1}{c|}{CS} & \multicolumn{1}{c|}{3.84} & \multicolumn{1}{c|}{1.56} & {-} & {-} & {-} & {-} & {***}\\
        \multicolumn{1}{c|}{OH} & \multicolumn{1}{c|}{5.73} & \multicolumn{1}{c|}{2.6} & {-} & {-} & {-} & {-} & {-}\\ 
        \midrule
    \multirow{2}{*}{\hspace{0.5cm}\vspace{-0.15cm}6m} & \multicolumn{3}{c|}{F(2.6, 49.9) = 10.4} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.354}\\ \cmidrule{2-8}
         & \multicolumn{1}{c|}{M} & {SD} & \multicolumn{1}{c|}{$p_{_{SR}}$}& \multicolumn{1}{c|}{$p_{_{SS}}$}& \multicolumn{1}{c|}{$p_{_{PS}}$}& \multicolumn{1}{c|}{$p_{_{CS}}$}& \multicolumn{1}{c}{$p_{_{OH}}$}\\ \midrule
        \multicolumn{1}{c|}{SR} & \multicolumn{1}{c|}{3.76} & \multicolumn{1}{c|}{1.24} & {-} & {ns}& {**} & {ns} & {***}\\
        \multicolumn{1}{c|}{SS} & \multicolumn{1}{c|}{3.60} & \multicolumn{1}{c|}{1.11} & {-} & {-} & {***} & {*} & {***}\\
        \multicolumn{1}{c|}{PS} & \multicolumn{1}{c|}{5.04} & \multicolumn{1}{c|}{2.04} & {-} & {-} & {-} & {*} & {ns}\\
        \multicolumn{1}{c|}{CS} & \multicolumn{1}{c|}{4.32} & \multicolumn{1}{c|}{1.51} & {-} & {-} & {-} & {-} & {**}\\
        \multicolumn{1}{c|}{OH} & \multicolumn{1}{c|}{5.33} & \multicolumn{1}{c|}{2.40} & {-} & {-} & {-} & {-} & {-}\\ 
        \midrule \midrule
\multicolumn{8}{c}{\textbf{Main effect}} \\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{\vspace{-0.15cm}Technique}} & \multicolumn{3}{c|}{F(4, 76) = 10.48} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.36}\\ \cmidrule{2-8}
& \multicolumn{1}{c|}{M} & {SD} & \multicolumn{1}{c|}{$p_{_{SR}}$}& \multicolumn{1}{c|}{$p_{_{SS}}$}& \multicolumn{1}{c|}{$p_{_{PS}}$}& \multicolumn{1}{c|}{$p_{_{CS}}$}& \multicolumn{1}{c}{$p_{_{OH}}$}\\ \midrule
\multicolumn{1}{c|}{SR} & {4.07} & {2.00} & {-} & {ns}& {**} & {*} & {***}\\
        \multicolumn{1}{c|}{SS} & {4.06} & {2.11} & {-} & {-} & {**} & {*} & {***}\\
        \multicolumn{1}{c|}{PS} & {5.20} & {2.48} & {-} & {-} & {-} & {ns} & {ns}\\
        \multicolumn{1}{c|}{CS} & {4.71} & {1.83} & {-} & {-} & {-} & {-} & {***}\\
        \multicolumn{1}{c|}{OH} & {5.87} & {2.58} & {-} & {-} & {-} & {-} & {-}\\ 
        \midrule
    \multicolumn{1}{l|}{\multirow{2}{*}{\vspace{-0.15cm}\hspace{0.1cm}Distance}} & \multicolumn{3}{c|}{F(1.6, 29.5) = 114.7} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.86}\\ \cmidrule{2-8}
& \multicolumn{1}{c|}{M} & {SD} &\multicolumn{1}{|c}{$p_{_{3m}}$}& \multicolumn{1}{|c}{$p_{_{6m}}$}& \multicolumn{1}{|c|}{$p_{_{9m}}$} \\ \midrule
        \multicolumn{1}{c|}{3m} & {3.71} & {1.98} & {-} & {***} & {***} \\
        \multicolumn{1}{c|}{6m} & {4.41} & {1.83} & {-} & {-} & {***}\\
        \multicolumn{1}{c|}{9m} & {6.22} & {2.34} & {-} & {-} & {-}\\
    \bottomrule
\end{tabular}
\label{table:ST_W_B}
\end{table}


\begin{table}
\centering
% \caption{With-Reference task: selection time results with the technique and distance conditions}
\caption{Task 1 - Error Distance results with ANOVA analysis. There is main effects on technique. M: Mean error distance (cm), SD: Standard Deviation, $p_{_{XX}}$: p-value for a comparison with XX, ns: not significant, $*$: $p$ \textless .05, $**$: $p$ \textless .01, $***$: $p$ \textless .001}
% \begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.5cm}| m{0.5cm} | m{1.6cm} | m{1.9cm}| m{2.2cm} | m{1.8cm}| m{1.5cm}}
\begin{tabular} {m{1.43cm} | m{0.7cm} | m{0.54cm} | m{0.457cm} | m{0.457cm}| m{0.457cm}| m{0.457cm}| m{0.457cm}}
\toprule 
\multicolumn{8}{c}{\textbf{Main effect}} \\ \midrule
    {\textbf{}} & \multicolumn{3}{c|}{\textbf{F}} & \multicolumn{2}{c|}{\textbf{$p$}} & \multicolumn{2}{c}{\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{\vspace{-0.15cm}Technique}} & \multicolumn{3}{c|}{F(4, 76) = 8.25} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.303}\\ \cmidrule{2-8}
& \multicolumn{1}{c|}{M} & {SD} & \multicolumn{1}{c|}{$p_{_{SR}}$}& \multicolumn{1}{c|}{$p_{_{SS}}$}& \multicolumn{1}{c|}{$p_{_{PS}}$}& \multicolumn{1}{c|}{$p_{_{CS}}$}& \multicolumn{1}{c}{$p_{_{OH}}$}\\ \midrule
\multicolumn{1}{c|}{SR} & {22.3} & {6.77} & {-} & {***}& {ns} & {**} & {**}\\
        \multicolumn{1}{c|}{SS} & {26.6} & {8.21} & {-} & {-} & {***} & {***} & {**}\\
        \multicolumn{1}{c|}{PS} & {20.4} & {7.32} & {-} & {-} & {-} & {ns} & {ns}\\
        \multicolumn{1}{c|}{CS} & {26.9} & {9.86} & {-} & {-} & {-} & {-} & {ns}\\
        \multicolumn{1}{c|}{OH} & {27.9} & {8.64} & {-} & {-} & {-} & {-} & {-}\\ 
        \midrule
    \bottomrule
\end{tabular}
\label{table:ED_W_B}
\end{table}

\begin{table*}[t]
\centering
% \caption{With-Reference task: selection time results with the technique and distance conditions}
\caption{Task 1 - NASA-TLX and UEQ results (Scales that have the main effect.)
The higher result indicates a worse result on effort and frustration level scales and a better result on attractiveness, efficiency, and dependability experience.}
% \begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.5cm}| m{0.5cm} | m{1.6cm} | m{1.9cm}| m{2.2cm} | m{1.8cm}| m{1.5cm}}
\begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.7cm}| m{0.5cm} | m{1.4cm} | m{1.4cm}| m{1.4cm} | m{1.4cm}| m{1.4cm}}
\toprule 
    {\textbf{Mean (SD)}} & {\textbf{F}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}} & {\textbf{Simple-Ray}}  & {\textbf{Simple-Stripe}} & {\textbf{Precision-Stripe}} & {\textbf{Cursor-Sync}} & {\textbf{One-Hand}}\\ \midrule
    % Interaction(T \texttimes D)  & {8, 152} & {7.247}  & {\textless .001} & {.276} \\ 
    % T  & {4, 76} &  {10.477}  & {\textless .001} & {.355} \\
    % D & {2, 38}  & {114.715} & {\textless .001} & {.858} \\
    Effort & {F(4, 76) = 3.24}& {.016}& {.146}& {3.30 (1.72)} & {3.55 (1.79)} & {2.80 (1.67)} & {2.70 (1.81)} & {3.75 (1.71)}\\ 
    Frustration Level & {F(2.56,48.75) = 5.29}& {.005}& {.218}& {2.85 (2.03)} & {2.80 (1.82)} & {1.65 (1.14)} & {1.90 (1.48)} & {2.60 (1.93)}\\ \midrule
    Attractiveness & {F(2.11, 40.07) = 3.34}& {.043}& {.149}& {0.62 (1.23)} & {0.90 (1.24)} & {1.30 (1.27)} & {1.42 (1.22)} & {0.61 (1.40)}\\ 
    Efficiency & {F(4, 76) = 3.38}& {.013}& {.151}& {1.23 (1.09)} & {1.05 (1.21)} & {1.60 (0.84)} & {1.74 (0.87)} & {0.85 (1.27)}\\ 
    Dependability & {F(4, 76) = 4.71}& {.002}& {.199}& {0.74 (1.02)} & {0.98 (1.19)} & {1.29 (0.87)} & {1.50 (1.01)} & {0.77 (0.97)}\\ 
    \bottomrule
\end{tabular}
\label{table:TLX_UEQ_W_B}
%\vspace{-0.6cm}
\end{table*}


% \begin{figure}[t]
% \centering
% \includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/TLX_with_box.pdf}
% % {ANOVA_Result_contents/figures/TLX_with_box.pdf}
% \caption{
% Task 1 - NASA-TLX result (95\% CI error bar):
% \dhk{
% Higher indicates worse (need more effort or be more frustrated) and lower indicates better (need less effort or be less frustrated).
% }
% } 
% \label{figure:TLX_W/R}   
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/UEQ_with_box.pdf}
% % {ANOVA_Result_contents/figures/UEQ_with_box.pdf}
% \caption{
% Task 1 - UEQ result (95\% CI error bar):
% \dhk{
% Higher indicates better experience and lower indicates worse experience.
% }
% } 
% \label{figure:UEQ_W/R}   
% \end{figure}

% The ANOVA results of selection time are reported in Figure \ref{figure:RT_W/R}.

The selection time results in Task 1 are reported in Figure \ref{figure:RT_W/R}.
There is an interaction effect between the technique and distance (F(8, 152) = 7.247, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .276).
Further analysis reveals that there are simple effects on technique at 3m (F(1.807, 34.336) = 24.627, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .564) and 6m (F(2.626, 49.890) = 10.394, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .354). However, there is no simple effect at 9m ($p$ = .164).
Pairwise comparisons reveal that, at the 3m target position, Simple-Ray has faster selection time (M = 2.75s, SD = 1.25) than Precision-Stripe (M = 3.69s, SD = 1.45, $p$ \textless .001), Cursor-Sync (M = 3.84s, SD = 1.56, $p$ = .002), and One-Hand (M = 5.73s, SD = 2.6, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 2.54s, SD = 0.89) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ = .002), and One-Hand ($p$ \textless .001). Furthermore, One-Hand has a significantly faster than Precision-Stripe ($p$ = .002) and Cursor-Sync ($p$ \textless .001).

At 6m, Simple-Ray has a faster selection time (M = 3.76s, SD = 1.24) than Precision-Stripe (M = 5.04s, SD = 2.04, $p$ = .002) and One-Hand (M = 5.33s, SD = 2.40, $p$ \textless .001).
Simple-Stripe also has a faster selection time (M = 3.60s, SD = 1.11) than Precision-Stripe ($p$ \textless .001), Cursor-Sync (M = 4.32s, SD = 1.51, $p$ = .027), and One-Hand ($p$ \textless .001).
Moreover, Cursor-Sync has a faster completion time than the Precision-Stripe ($p$ = .033) and One-Hand ($p$ = .008).

There is a main effects on technique (F(4, 76) = 10.480, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .36).
Pairwise comparisons show that Simple-Ray (M = 4.07s, SD = 2.00) has a faster selection time than Precision-Stripe (M = 5.20s, SD = 2.48, $p$ = .004), Cursor-Sync (M = 4.71s, SD = 1.83, $p$ = .042), and One-Hand (M = 5.87s, SD = 2.58, $p$ \textless .001).
In addition, Simple-Stripe also results (M = 4.06s, SD = 2.11) faster than Precision-Stripe ($p$ = .009), Cursor-Sync ($p$ = .044), and One-Hand ($p$ \textless .001).
Moreover, Cursor-Sync is significantly faster than One-Hand ($p$ \textless .001).

A significant main effect is found on distance (F(1.552, 29.496) = 114.720, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .86).
Pairwise comparisons reveal that 3m (M = 3.71s, SD = 1.98) has a faster selection time than 6m (M = 4.41s, SD = 1.83, $p$ \textless .001) and 9m (M = 6.22s, SD = 2.34, $p$ \textless .001).
In addition, 6m is faster than 9m ($p$ \textless .001).
These results partially support \textbf{H1} and \textbf{H2}.




\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/error_distance_with_box.pdf}
% {ANOVA_Result_contents/figures/error_distance_with_box.pdf}
\caption{
Task 1 - Error Distance results with 95\% CI:
\dhk{Lower values indicate accurate performance, while
higher values are inaccurate. 
}
} 
\label{figure:ED_W/R}
\end{figure}

\subsubsection{Error Distance}

The results are reported in Figure \ref{figure:ED_W/R}.
A significant main effect is found on technique (F(4, 76) = 8.251, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .303).
Pairwise comparisons show that Simple-Ray has a smaller error distance (M = 22.26cm, SD = 6.77) than Simple-Stripe (M = 26.6cm, SD = 8.21, $p$ \textless .001), Cursor-Sync (M = 26.86cm, SD = 9.86, $p$ = .005), and One-Hand (M = 27.91cm, SD = 8.64, $p$ = .003).
In addition, Precision-Stripe has a significantly lower error distance (M = 20.35cm, SD = 7.32) than Simple-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ = .002).
These results do not support \textbf{H3} and \textbf{H4}.

% \subsubsection{Button Clicks}
% The results of the number of button clicks are reported in Figure \ref{figure:AT_W/R}. % and Table [].
% There is an interaction effect between technique and  distance (F(3.476, 66.041) = 16.239, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .461).
% Further analysis reveals that there are simple effects on technique at 6m (F(1.836, 34.879) = 4.563, $p$ = .020, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = 194) and 9m (F(2.465,46.831) = 23.826, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .556).
% Pairwise comparisons reveal that, at the 6m target position, Simple-Ray has more button clicks (M = 1.60, SD = 1.00) than Cursor-Sync (M = 1.03, SD = 0.11, $p$ = .012) and One-Hand Simultaneous (M = 1.03, SD = 0.11, $p$ = .020).
% In addition, Simple-Stripe leads to more button clicks (M = 1.50, SD = 0.63) than Cursor-Sync ($p$ = .001) and One-Hand Simultaneous ($p$ = .004).

% At 9m, Simple-Ray has more button clicks (M = 2.65, SD = 1.26) than Precision-Stripe (M = 1.58, SD = 0.82, $p$ = .002), Cursor-Sync (M = 1.08, SD = 0.34, $p$ < .001), and One-Hand Simultaneous (M = 1.00, SD = 0.00, $p$ < .001).
% In addition, Simple-Stripe (M = 3.10, SD = 1.35) has more button clicks than Precision-Stripe ($p$ = .002), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).

% There are main effects on technique (F(2.111, 40.113) = 18.430, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .492) and distance (F(1.403, 26.658) = 67.413, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .780).
% Pairwise comparisons show that Simple-Ray has more button clicks (M = 1.79, SD = 1.13) than Precision-Stripe (M = 1.28, SD = 0.60, $p$ = .011), Cursor-Sync (M = 1.05, SD = 0.24, $p$ \textless .001), and One-Hand Simultaneous (M = 1.04, SD = 0.21, $p$ \textless .001).
% In addition, Simple-Stripe (M = 1.89, SD = 1.23) has more button clicks than Precision-Stripe ($p$ = .002), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).
% Furthermore, Precision-Stripe has more attempts than Cursor-Sync ($p$ = .029) and One-Hand Simultaneous ($p$ = .008).

% Pairwise comparisons show that 3m (M = 1.08, SD = 0.27) has more button clicks than 6m (M = 1.28, SD = 0.62, $p$ \textless .001) and 9m (M = 1.88. SD = 1.24, $p$ < .001). In addition, 6m has more button clicks than 9m ($p$ \textless .001).


\subsubsection{NASA-TLX}

The NASA-TLX results are presented in the upper part of Table \ref{table:TLX_UEQ_W_B}.

\paragraph{Effort}
There is a main effect on Effort ($p$ = .016).
A pairwise comparison shows that Precision-Stripe has a lower effort rate than Simple-Stripe ($p$ = .014) and One-Hand ($p$ = .016).
In addition, Cursor-Sync has a lower Effort rate than Simple-Stripe ($p$ = .034) and One-Hand ($p$ = .018).

\paragraph{Frustration}
A main effect on Frustration ($p$ = .005) is found.
Pairwise comparisons reveal that Precision-Stripe has a lower value than Simple-Ray ($p$ = .006), Simple-Stripe ($p$ = .003), Cursor-Sync ($p$ = .016), and One-Hand ($p$ = .040).
In addition, Cursor-Sync has a lower Frustration rate than Simple-Ray ($p$ = .040).

There are no significant main effects on Mental Demand, Physical Demand, Performance, and Temporal Demand on technique.
\dhk{
These results are partially support our hypothesis (\textbf{H5}).
}

\subsubsection{UEQ}
The results of the UEQ are presented in the lower part of Table \ref{table:TLX_UEQ_W_B}.
\paragraph{Attractiveness}
There is a main effect on Attractiveness ($p$ = .043).
Pairwise comparisons show that Cursor-Sync has a higher value than Simple-Ray ($p$ = .021) and Simple-Stripe ($p$ = .047).

\paragraph{Efficiency}
There is a main effect on Efficiency ($p$ = .013).
Cursor-Sync has higher Efficiency rate than Simple-Stripe ($p$ = .037) and One-Hand ($p$ = .020).
In addition, Precision-Stripe has a higher Efficiency rate than One-Hand ($p$ = .036).

\paragraph{Dependability}
There is a main effect on Dependability ($p$ = .002). 
Comparisons show that Precision-Stripe has a higher Dependability rate than Simple-Ray ($p$ = .036) and One-Hand ($p$ = .023).
In addition, Cursor-Sync has a higher Dependability rate than Simple-Ray ($p$ = .005), Simple-Stirpe ($p$ = .032), and One-Hand ($p$ = .006).

There is no significant difference in Novelty, Perspicuity, and Stimulation among techniques.
These results are partially support our hypothesis (\textbf{H5}).

\subsection{Results: Task 2 \dhk{- \textit{without Reference}}}
\subsubsection{Selection Time}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/selection_time_without_box.pdf}
% {ANOVA_Result_contents/figures/response_time_without_box.pdf}
\caption{
% Task 2 - Selection Time result: Selection time results for each technique and distance (95\% CI error bar).
Task 2 - Selection Time results with 95\% CI.
\dhk{
Lower values indicate better/faster performance, whereas higher values signify poorer performance.
}
} 
\label{figure:RT_O/R}   
\end{figure}

The selection time results in Task 2 with each condition are reported in Figure \ref{figure:RT_O/R}.
These results show an interaction effect between the technique type and the target position distance (F(8, 152) = 13.324, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .412).
Further analysis reveals that there are simple effects on technique at 3m (F(1.944, 36.929) = 72.526, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .792), 6m (F(4, 76) = 49.594, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .723), and 9m (F(4, 76) = 59.515, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .758).
Pairwise comparisons reveal that, at the 3m target position, Simple-Ray has faster selection time (M = 1.71s, SD = 0.73) than Precision-Stripe (M = 2.90s, SD = 0.77, $p$ \textless .001), Cursor-Sync (M = 2.52s, SD = 0.73, $p$ \textless .001), and One-Hand (M = 5.05s, SD = 1.46, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 1.88s, SD = 0.60) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ \textless .001).
Furthermore, Precision-Stripe has a significantly faster selection than One-Hand ($p$ \textless .001).
Lastly, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .037) and One-Hand ($p$ \textless .001).

At 6m, Simple-Ray has faster selection time (M = 2.13s, SD = 1.06) than Precision-Stripe (M = 4.19s, SD = 1.39, $p$ \textless .001), Cursor-Sync (M = 3.47s, SD = 1.06, $p$ \textless .001), and One-Hand (M = 4.67s, SD = 1.39, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 2.35s, SD = 0.63) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ \textless .001).
Furthermore, Precision-Stripe has a significantly faster selection than One-Hand ($p$ = .037).
Lastly, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .014) and One-Hand ($p$ \textless .001).

At 9m, Simple-Ray has faster selection time (M = 2.41s, SD = 1.22) than Precision-Stripe (M = 5.22s, SD = 1.92, $p$ \textless .001), Cursor-Sync (M = 4.39s, SD = 1.37, $p$ \textless .001), and One-Hand (M = 5.44s, SD = 1.45, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 2.60s, SD = 0.71) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ \textless .001).
Furthermore, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .011) and One-Hand ($p$ \textless .001).

There are main effects on technique (F(4, 76) = 88.065, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .823) and distance (F(2, 38) = 56.226, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .747).

Pairwise comparisons show that Simple-Ray (M = 2.08s, SD = 1.05) has a faster selection time than Precision-Stripe (M = 4.11s, SD = 1.71, $p$ \textless .001), Cursor-Sync (M = 3.46s, SD = 1.31, $p$ \textless .001), and One-Hand (M = 5.05s, SD = 1.45, $p$ \textless .001).
In addition, Simple-Stripe has a faster result (M = 2.28s, SD = 0.71) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ \textless .001)
Furthermore, Simple-Stripe has a faster completion time than One-Hand ($p$ \textless .001), and Cursor-Sync has a faster completion time than Precision-Stripe ($p$ = .008) and One-Hand ($p$ \textless .001).

Pairwise comparisons show that 3m (M = 2.81s, SD = 1.50) is faster than 6m (M = 3.36s, SD = 1.50, $p$ \textless .001) and 9m (M = 4.01s, SD = 1.87, $p$ \textless .001).
In addition, 6m is faster than  9m ($p$ \textless .001).
These results support \textbf{H1} and \textbf{H2}.

\subsubsection{Error Distance}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/error_distance_without_box.pdf}
% {ANOVA_Result_contents/figures/error_distance_without_box.pdf}
\caption{
Task 2 - Error Distance results with 95\% CI:
\dhk{
Lower values indicate accurate performance, while
higher values are inaccurate. 
% Higher indicates worse performance (inaccurate) and lower indicates better performance (accurate).
}
} 
\label{figure:ED_O/R}   
\end{figure}


\begin{table}
\centering
% \caption{With-Reference task: selection time results with the technique and distance conditions}
\caption{Task 2 - Selection Time results with ANOVA analysis. There are interaction effects at 3m and 6m and main effects on technique and distance. M: Mean selection time (s), SD: Standard Deviation, $p_{_{XX}}$: p-value for a comparison with XX, ns: not significant, $*$: $p$ \textless .05, $**$: $p$ \textless .01, $***$: $p$ \textless .001}
% \begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.5cm}| m{0.5cm} | m{1.6cm} | m{1.9cm}| m{2.2cm} | m{1.8cm}| m{1.5cm}}
\begin{tabular} {m{1.43cm} | m{0.7cm} | m{0.54cm} | m{0.457cm} | m{0.457cm}| m{0.457cm}| m{0.457cm}| m{0.457cm}}
\toprule 
\multicolumn{8}{c}{\textbf{Interaction effect}} \\ \midrule
    {\textbf{}} & \multicolumn{3}{c|}{\textbf{F}} & \multicolumn{2}{c|}{\textbf{$p$}} & \multicolumn{2}{c}{\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
    \multicolumn{1}{l|}{{Interaction}} & \multicolumn{3}{c|}{F(8, 152) = 7.25}    &   \multicolumn{2}{c|}{***}    &   \multicolumn{2}{c}{.276}\\ \midrule \midrule
    \multirow{2}{*}{\hspace{0.5cm}\vspace{-0.15cm}3m} & \multicolumn{3}{c|}{F(1.8, 34.3) = 24.6} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.564}\\ \cmidrule{2-8}
         & \multicolumn{1}{c|}{M} & \multicolumn{1}{c|}{SD} & \multicolumn{1}{c|}{$p_{_{SR}}$}& \multicolumn{1}{c|}{$p_{_{SS}}$}& \multicolumn{1}{c|}{$p_{_{PS}}$}& \multicolumn{1}{c|}{$p_{_{CS}}$}& \multicolumn{1}{c}{$p_{_{OH}}$}\\ \midrule
        \multicolumn{1}{c|}{SR} & \multicolumn{1}{c|}{2.75} & \multicolumn{1}{c|}{1.25} & {-} & {ns}& {***} & {**} & {***}\\
        \multicolumn{1}{c|}{SS} & \multicolumn{1}{c|}{2.54} & \multicolumn{1}{c|}{0.89} & {-} & {-} & {***} & {**} & {***}\\
        \multicolumn{1}{c|}{PS} & \multicolumn{1}{c|}{3.69} & \multicolumn{1}{c|}{1.45} & {-} & {-} & {-} & {ns} & {**}\\
        \multicolumn{1}{c|}{CS} & \multicolumn{1}{c|}{3.84} & \multicolumn{1}{c|}{1.56} & {-} & {-} & {-} & {-} & {***}\\
        \multicolumn{1}{c|}{OH} & \multicolumn{1}{c|}{5.73} & \multicolumn{1}{c|}{2.6} & {-} & {-} & {-} & {-} & {-}\\ 
        \midrule
    \multirow{2}{*}{\hspace{0.5cm}\vspace{-0.15cm}6m} & \multicolumn{3}{c|}{F(2.6, 49.9) = 10.4} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.354}\\ \cmidrule{2-8}
         & \multicolumn{1}{c|}{M} & {SD} & \multicolumn{1}{c|}{$p_{_{SR}}$}& \multicolumn{1}{c|}{$p_{_{SS}}$}& \multicolumn{1}{c|}{$p_{_{PS}}$}& \multicolumn{1}{c|}{$p_{_{CS}}$}& \multicolumn{1}{c}{$p_{_{OH}}$}\\ \midrule
        \multicolumn{1}{c|}{SR} & \multicolumn{1}{c|}{3.76} & \multicolumn{1}{c|}{1.24} & {-} & {ns}& {**} & {ns} & {***}\\
        \multicolumn{1}{c|}{SS} & \multicolumn{1}{c|}{3.60} & \multicolumn{1}{c|}{1.11} & {-} & {-} & {***} & {*} & {***}\\
        \multicolumn{1}{c|}{PS} & \multicolumn{1}{c|}{5.04} & \multicolumn{1}{c|}{2.04} & {-} & {-} & {-} & {*} & {ns}\\
        \multicolumn{1}{c|}{CS} & \multicolumn{1}{c|}{4.32} & \multicolumn{1}{c|}{1.51} & {-} & {-} & {-} & {-} & {**}\\
        \multicolumn{1}{c|}{OH} & \multicolumn{1}{c|}{5.33} & \multicolumn{1}{c|}{2.40} & {-} & {-} & {-} & {-} & {-}\\ 
        \midrule \midrule
\multicolumn{8}{c}{\textbf{Main effect}} \\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{\vspace{-0.15cm}Technique}} & \multicolumn{3}{c|}{F(4, 76) = 10.48} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.36}\\ \cmidrule{2-8}
& \multicolumn{1}{c|}{M} & {SD} & \multicolumn{1}{c|}{$p_{_{SR}}$}& \multicolumn{1}{c|}{$p_{_{SS}}$}& \multicolumn{1}{c|}{$p_{_{PS}}$}& \multicolumn{1}{c|}{$p_{_{CS}}$}& \multicolumn{1}{c}{$p_{_{OH}}$}\\ \midrule
\multicolumn{1}{c|}{SR} & {4.07} & {2.00} & {-} & {ns}& {**} & {*} & {***}\\
        \multicolumn{1}{c|}{SS} & {4.06} & {2.11} & {-} & {-} & {**} & {*} & {***}\\
        \multicolumn{1}{c|}{PS} & {5.20} & {2.48} & {-} & {-} & {-} & {ns} & {ns}\\
        \multicolumn{1}{c|}{CS} & {4.71} & {1.83} & {-} & {-} & {-} & {-} & {***}\\
        \multicolumn{1}{c|}{OH} & {5.87} & {2.58} & {-} & {-} & {-} & {-} & {-}\\ 
        \midrule
    \multicolumn{1}{l|}{\multirow{2}{*}{\vspace{-0.15cm}\hspace{0.1cm}Distance}} & \multicolumn{3}{c|}{F(1.6, 29.5) = 114.7} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.86}\\ \cmidrule{2-8}
& \multicolumn{1}{c|}{M} & {SD} &\multicolumn{1}{|c}{$p_{_{3m}}$}& \multicolumn{1}{|c}{$p_{_{6m}}$}& \multicolumn{1}{|c|}{$p_{_{9m}}$} \\ \midrule
        \multicolumn{1}{c|}{3m} & {3.71} & {1.98} & {-} & {***} & {***} \\
        \multicolumn{1}{c|}{6m} & {4.41} & {1.83} & {-} & {-} & {***}\\
        \multicolumn{1}{c|}{9m} & {6.22} & {2.34} & {-} & {-} & {-}\\
    \bottomrule
\end{tabular}
\label{table:ST_Without_B}
\end{table}


\begin{table}
\centering
% \caption{With-Reference task: selection time results with the technique and distance conditions}
\caption{Task 2 - Error Distance results with ANOVA analysis. There is main effects on technique. M: Mean error distance (cm), SD: Standard Deviation, $p_{_{XX}}$: p-value for a comparison with XX, ns: not significant, $*$: $p$ \textless .05, $**$: $p$ \textless .01, $***$: $p$ \textless .001}
% \begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.5cm}| m{0.5cm} | m{1.6cm} | m{1.9cm}| m{2.2cm} | m{1.8cm}| m{1.5cm}}
\begin{tabular} {m{1.43cm} | m{0.7cm} | m{0.54cm} | m{0.457cm} | m{0.457cm}| m{0.457cm}| m{0.457cm}| m{0.457cm}}
\toprule 
\multicolumn{8}{c}{\textbf{Main effect}} \\ \midrule
    {\textbf{}} & \multicolumn{3}{c|}{\textbf{F}} & \multicolumn{2}{c|}{\textbf{$p$}} & \multicolumn{2}{c}{\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{\vspace{-0.15cm}Technique}} & \multicolumn{3}{c|}{F(4, 76) = 8.25} & \multicolumn{2}{c|}{***} & \multicolumn{2}{c}{.303}\\ \cmidrule{2-8}
& \multicolumn{1}{c|}{M} & {SD} & \multicolumn{1}{c|}{$p_{_{SR}}$}& \multicolumn{1}{c|}{$p_{_{SS}}$}& \multicolumn{1}{c|}{$p_{_{PS}}$}& \multicolumn{1}{c|}{$p_{_{CS}}$}& \multicolumn{1}{c}{$p_{_{OH}}$}\\ \midrule
\multicolumn{1}{c|}{SR} & {22.3} & {6.77} & {-} & {***}& {ns} & {**} & {**}\\
        \multicolumn{1}{c|}{SS} & {26.6} & {8.21} & {-} & {-} & {***} & {***} & {**}\\
        \multicolumn{1}{c|}{PS} & {20.4} & {7.32} & {-} & {-} & {-} & {ns} & {ns}\\
        \multicolumn{1}{c|}{CS} & {26.9} & {9.86} & {-} & {-} & {-} & {-} & {ns}\\
        \multicolumn{1}{c|}{OH} & {27.9} & {8.64} & {-} & {-} & {-} & {-} & {-}\\ 
        \midrule
    \bottomrule
\end{tabular}
\label{table:ED_Without_B}
\end{table}

\begin{table*}[t]
\centering
% \caption{With-Reference task: selection time results with the technique and distance conditions}
\caption{Task 2 - NASA-TLX and UEQ results (Scales that have the main effect.)
The higher result indicates a worse result on mental demand and effort and a better result on performance, attractiveness, efficiency, perspicuity, dependability, and stimulation.
}
\begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.7cm}| m{0.5cm} | m{1.4cm} | m{1.4cm}| m{1.4cm} | m{1.4cm}| m{1.4cm}}
\toprule 
    {\textbf{Mean (SD)}} & {\textbf{F}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}} & {\textbf{Simple-Ray}}  & {\textbf{Simple-Stripe}} & {\textbf{Precision-Stripe}} & {\textbf{Cursor-Sync}} & {\textbf{One-Hand}}\\ \midrule
% \begin{tabular} {m{2.2cm} | m{1.8cm} | m{2.0cm}| m{2.2cm} | m{1.8cm}| m{1.6cm}}
% \toprule 
    % {\textbf{Mean (SD)}} & {\textbf{Simple-Ray}}  & {\textbf{Simple-Stripe}} & {\textbf{Precision-Stripe}} & {\textbf{Cursor-Sync}} & {\textbf{One-Hand}}\\ \midrule
    % Interaction(T \texttimes D)  & {8, 152} & {7.247}  & {\textless .001} & {.276} \\ 
    % T  & {4, 76} &  {10.477}  & {\textless .001} & {.355} \\
    % D & {2, 38}  & {114.715} & {\textless .001} & {.858} \\
    Mental Demand & {F(3.07, 58.34) = 4.57} & {.006} & {.194} & {3.15 (1.66)} & {2.85 (1.79)} & {3.00 (1.69)} & {3.10 (1.97)} & {4.25 (1.94)}\\ 
    Performance & {F(4, 76) = 7.46} & {\textless .001} & {.282} & {4.85 (1.76)} & {4.95 (1.61)} & {5.35 (1.57)} & {4.80 (1.61)} & {3.65 (1.50)}\\
    Effort & {F(4, 76) = 5.15} & {\textless .001} & {.213} & {3.25 (1.89)} & {2.80 (1.40)} & {3.25 (1.80)} & {2.75 (1.68)} & {4.00 (1.89)}\\ \midrule
    Attractiveness & {F(2.39, 45.32) = 8.37} & {\textless .001} & {.306} & {1.18 (1.11)} & {1.14 (1.51)} & {1.58 (1.12)} & {1.31 (1.16)} & {0.18 (1.57)}\\ 
    Efficiency & {F(2.30, 43.79) = 5.42} & {.006} & {.222} & {1.59 (0.80)} & {1.58 (1.11)} & {1.75 (0.86)} & {1.81 (0.97)} & {0.79 (1.24)}\\ 
    Perspicuity & {F(2.49, 47.23) = 6.42} & {.002} & {.253} & {2.31 (0.81)} & {2.04 (1.28)} & {2.11 (1.02)} & {2.00 (1.23)} & {1.10 (1.32)}\\
    Dependability & {F(2.22, 42.17) = 6.89} & {.002} & {.266} & {1.09 (0.94)} & {1.24 (0.88)} & {1.39 (0.84)} & {1.33 (0.97)} & {0.37 (1.21)}\\
    Stimulation & {F(4, 76) = 4.26} & {.004} & {.183} & {0.86 (1.23)} & {0.88 (1.48)} & {1.21 (1.19)} & {1.20 (0.97)} & {0.23 (1.34)}\\
    \bottomrule
\end{tabular}
\label{table:TLX_UEQ_Without_B}
%\vspace{-0.6cm}
\end{table*}

The error distance results with each condition are reported in Figure \ref{figure:ED_O/R}.
There is an interaction effect between technique and target position distance (F(8, 152) = 11.634, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .380).
Further examination shows significant simple effects of the techniques at distances of 3m (F(2.505, 47.596) = 24.371, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .562), 6m (F(4, 76) = 12.079, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .389), and 7m (F(1.755, 33.350) = 9.300, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .329).



Pairwise comparisons show that, with a 3m located target, One-Hand (M = 50.60cm, SD = 21.37, $p$ \textless .001) has significantly lower accurate rates than Simple-Ray (M = 22.50cm, SD = 14.30), Simple-Stripe (M = 17.61cm, SD = 9.25),  Precision-Stripe (M = 18.80cm, SD = 14.69) and Cursor-Sync (M = 14.83cm, SD = 7.37).
In addition, Simple-Ray is less accurate than the Cursor-Sync ($p$ = .041) technique.

With a 6m condition,  Simple-Stripe has more accurate results (M = 51.68cm, SD = 23.42) than Simple-Ray (M = 70.58cm, SD = 40.13, $p$ = .025) and One-Hand (M = 91.70cm, SD = 49.75, $p$ = .001).
Precision-Stripe is also more accurate (M = 42.04cm, SD = 34.58) than Simple-Ray ($p$ = .002) and One-Hand ($p$ \textless .001). 
Moreover, Cursor-Sync is more accurate (M = 32.72cm, SD = 19.74) than Simple-Ray ($p$ \textless .001), Simple-Stripe ($p$ = .014), and One-Hand ($p$ \textless .001) techniques.

With a 9m condition, Simple-Ray is less accurate (M = 161.01cm, SD = 117.66) than Precision-Stripe (M = 77.78cm, SD = 32.08, $p$ = .002), Cursor-Sync (M = 66.33cm, SD = 35.23, $p$ \textless .001), and One-Hand (M = 71.42cm, SD = 32.26, $p$ = .006).
Simple-Stripe technique is also less accurate (M = 114.71cm, SD = 45.74) than Precision-Stripe ($p$ = .013), Cursor-Sync ($p$ = .003), and One-Hand ($p$ = .001).

There are main effects on technique (F(4, 76) = 9.294, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .328) and distance (F(2, 38) = 90.853, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .827). 
Pairwise comparisons show that Precision-Stripe has a less error distance (M = 46.21cm, SD = 37.21) than Simple-Ray (M = 84.70cm, SD = 91.63, $p$ \textless .001) and One-Hand (M = 71.24cm, SD = 39.57, $p$ = .002).
In addition, Cursor-Sync has a less error distance (M = 37.96cm, SD = 31.72) than Simple-Ray ($p$ \textless .001), Simple-Stripe (M = 61.34cm, SD = 50.23, $p$ = .004), Precision-Stripe ($p$ = .046), and One-Hand ($p$ \textless .001).
Lastly, the participants complete the task more accurately when a target position is 3m (M = 24.87cm, SD = 19.20) than 6m (M = 57.74cm, SD = 40.54, $p$ \textless .001) and 9m (M = 98.25cm, SD = 70.57, $p$ \textless .001), and also, the result from 6m is more accurate than from 9m ($p$ \textless .001).
\dhk{
These results partially support \textbf{H3} and \textbf{H4}.
}
\subsubsection{NASA-TLX}

% \begin{figure}[t]
% \centering
% \includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/TLX_without_box.pdf}
% % {ANOVA_Result_contents/figures/TLX_without_box.pdf}
% \caption{
% Task 2 - NASA-TLX result (95\% CI error bar):
% \dhk{
% Higher indicates worse and lower indicates better workload for mental demand and effort.
% In contrast, for performance, higher indicates better, and lower indicates worse.
% }
% } 
% \label{figure:TLX_O/R}   
% \end{figure}

The NASA-TLX results are shown in the upper part of the Table \ref{table:TLX_UEQ_Without_B}.

\paragraph{Mental Demand}
There is a main effect on Mental Demand ($p$ = .006).
Pairwise comparisons show that One-Hand has a higher Mental Demand rate than Simple-Ray ($p$ = .005), Simple-Stripe ($p$ = .001), Precision-Stripe ($p$ = .008), and Cursor-Sync ($p$ = .012).

\paragraph{Performance}
 In addition, there is a significant main effect on Performance ($p$ \textless .001).
 One-Hand has lower performance rate than Simple-Ray ($p$ \textless .001), Simple-Stripe ($p$ \textless .001), Precision-Stripe ($p$ \textless .001), and Cursor-Sync ($p$ \textless .001).

\paragraph{Effort}
There is a main effect on Effort ($p$ \textless .001).
One-Hand has higher Effort rate than Simple-Ray ($p$ = .021), Simple-Stripe ($p$ = .006), and Cursor-Sync ($p$ = .002).
However, there is no difference between One-Hand and Precision-Stripe, and among Simple-Ray, Simple-Stripe, and Cursor-Sync.

There is no significant main effect on Frustration, Physical Demand, and Temporal Demand.
\dhk{
These results are partially support our hypothesis (\textbf{H5}).
}
\subsubsection{UEQ}

% \begin{figure}[t]
% \centering
% \includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/UEQ_without_box.pdf}
% % {ANOVA_Result_contents/figures/UEQ_without_box.pdf}
% \caption{
% Task 2 - UEQ result (95\% CI error bar):
% \dhk{
% Higher indicates better experience and lower indicates worse experience.
% }
% } 
% \label{figure:UEQ_O/R}   
% \end{figure}

The UEQ results are presented in the bottom part of the Table \ref{table:TLX_UEQ_Without_B}.

\paragraph{Attractiveness}
There is a main effect on Attractiveness ($p$ \textless .001).
Pairwise comparisons show that One-Hand has a lower Attractiveness rate than Simple-Ray ($p$ \textless .001), Simple-Stripe ($p$ = .012), Precision-Stripe ($p$ \textless .001), and Cursor-Sync ($p$ = .003).
In addition, Simple-Stripe has a lower Attractiveness rate than Precision-Stripe ($p$ = .022).

\paragraph{Efficiency}
There is a main effect on Efficiency ($p$ = .006).
One-Hand has a lower Efficiency rate than Simple-Ray ($p$ = .011), Simple-Stripe ($p$ = .039), Precision-Stripe ($p$ = .005), and Cursor-Sync ($p$ = .008).

\paragraph{Perspicuity}
There is a main effect on Perspicuity ($p$ = .002).
One-Hand has a lower perspicuity rate than Simple-Ray ($p$ \textless .001),  Simple-Stripe ($p$ = .007), Precision-Stripe ($p$ = .002), and Cursor-Sync ($p$ = .026).

\paragraph{Dependability}
Moreover, there is a main effect on Dependability ($p$ = .002).
One-Hand has a lower Dependability rate than Simple-Ray ($p$ = .029), Simple-Stripe ($p$ = .005), Precision-Stripe ($p$ = .002), and Cursor-Sync ($p$ = .006). 

\paragraph{Stimulation}
Lastly, there is a main effect on Stimulation ($p$ = .004).
One-Hand has a lower Stimulation rate than Simple-Ray ($p$ = .020), Precision-Stripe ($p$ = .011) and Cursor-Sync ($p$ = .006).
However, there is no significant difference between One-Hand and Simple-Stripe.

The Novelty of each technique is not significantly different in this task.
\dhk{
These results are partially support our hypothesis (\textbf{H5}).
}

==> ANOVA_Result_contents/4_result_short.tex <==
\section{Result}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/selection_time_with_box.pdf}
% {ANOVA_Result_contents/figures/response_time_with_box.pdf}
\caption{
Task 1 - Selection Time results with 95\% CI:
\dhk{
Lower values indicate better/faster performance, whereas higher values signify poorer performance.
% Higher indicates worse performance (delayed) and lower indicates better performance (quick).
}
} 
\label{figure:RT_W/R}   
\end{figure}



This section reports the study results.
We utilized a two-way repeated measures Analysis of Variance (ANOVA) test, with a significance level of 5\%, to analyze selection time, error distance, and user experience responses (measured by NASA-TLX and UEQ) for each task. Additionally, we applied the Geisser-Greenhouse correction to guard against potential violations of the sphericity assumption.
The post-hoc test is conducted by Fisher's least significant differences (LSD) pairwise comparison with $\alpha$ = .05 level for significance.
We employ the median as the representative value for our analysis to mitigate the potential skewness of the collected data.

% \subsection{Task 1 Results}
\subsection{Result: Task 1 \dhk{- \textit{with Reference}}}

\subsubsection{Selection Time}




\begin{table*}[t]
\centering
% \caption{With-Reference task: selection time results with the technique and distance conditions}
\caption{Task 1 - NASA-TLX and UEQ results (Scales that have the main effect.)
The higher result indicates a worse result on effort and frustration level scales and a better result on attractiveness, efficiency, and dependability experience.}
% \begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.5cm}| m{0.5cm} | m{1.6cm} | m{1.9cm}| m{2.2cm} | m{1.8cm}| m{1.5cm}}
\begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.7cm}| m{0.5cm} | m{1.4cm} | m{1.4cm}| m{1.4cm} | m{1.4cm}| m{1.4cm}}
\toprule 
    {\textbf{Mean (SD)}} & {\textbf{F}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}} & {\textbf{Simple-Ray}}  & {\textbf{Simple-Stripe}} & {\textbf{Precision-Stripe}} & {\textbf{Cursor-Sync}} & {\textbf{One-Hand}}\\ \midrule
    % Interaction(T \texttimes D)  & {8, 152} & {7.247}  & {\textless .001} & {.276} \\ 
    % T  & {4, 76} &  {10.477}  & {\textless .001} & {.355} \\
    % D & {2, 38}  & {114.715} & {\textless .001} & {.858} \\
    Effort & {F(4, 76) = 3.24}& {.016}& {.146}& {3.30 (1.72)} & {3.55 (1.79)} & {2.80 (1.67)} & {2.70 (1.81)} & {3.75 (1.71)}\\ 
    Frustration Level & {F(2.56,48.75) = 5.29}& {.005}& {.218}& {2.85 (2.03)} & {2.80 (1.82)} & {1.65 (1.14)} & {1.90 (1.48)} & {2.60 (1.93)}\\ \midrule
    Attractiveness & {F(2.11, 40.07) = 3.34}& {.043}& {.149}& {0.62 (1.23)} & {0.90 (1.24)} & {1.30 (1.27)} & {1.42 (1.22)} & {0.61 (1.40)}\\ 
    Efficiency & {F(4, 76) = 3.38}& {.013}& {.151}& {1.23 (1.09)} & {1.05 (1.21)} & {1.60 (0.84)} & {1.74 (0.87)} & {0.85 (1.27)}\\ 
    Dependability & {F(4, 76) = 4.71}& {.002}& {.199}& {0.74 (1.02)} & {0.98 (1.19)} & {1.29 (0.87)} & {1.50 (1.01)} & {0.77 (0.97)}\\ 
    \bottomrule
\end{tabular}
\label{table:TLX_UEQ_W_B}
%\vspace{-0.6cm}
\end{table*}


% \begin{figure}[t]
% \centering
% \includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/TLX_with_box.pdf}
% % {ANOVA_Result_contents/figures/TLX_with_box.pdf}
% \caption{
% Task 1 - NASA-TLX result (95\% CI error bar):
% \dhk{
% Higher indicates worse (need more effort or be more frustrated) and lower indicates better (need less effort or be less frustrated).
% }
% } 
% \label{figure:TLX_W/R}   
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/UEQ_with_box.pdf}
% % {ANOVA_Result_contents/figures/UEQ_with_box.pdf}
% \caption{
% Task 1 - UEQ result (95\% CI error bar):
% \dhk{
% Higher indicates better experience and lower indicates worse experience.
% }
% } 
% \label{figure:UEQ_W/R}   
% \end{figure}

% The ANOVA results of selection time are reported in Figure \ref{figure:RT_W/R}.
The selection time results in Task 1 are reported in Figure \ref{figure:RT_W/R}.
There is an interaction effect between the technique and distance (F(8, 152) = 7.247, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .276).
Further analysis reveals that there are simple effects on technique at 3m (F(1.807, 34.336) = 24.627, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .564) and 6m (F(2.626, 49.890) = 10.394, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .354). However, there is no simple effect at 9m ($p$ = .164).
Pairwise comparisons reveal that, at the 3m target position, Simple-Ray has faster selection time (M = 2.75s, SD = 1.25) than Precision-Stripe (M = 3.69s, SD = 1.45, $p$ \textless .001), Cursor-Sync (M = 3.84s, SD = 1.56, $p$ = .002), and One-Hand (M = 5.73s, SD = 2.6, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 2.54s, SD = 0.89) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ = .002), and One-Hand ($p$ \textless .001). Furthermore, One-Hand has a significantly faster than Precision-Stripe ($p$ = .002) and Cursor-Sync ($p$ \textless .001).

At 6m, Simple-Ray has a faster selection time (M = 3.76s, SD = 1.24) than Precision-Stripe (M = 5.04s, SD = 2.04, $p$ = .002) and One-Hand (M = 5.33s, SD = 2.40, $p$ \textless .001).
Simple-Stripe also has a faster selection time (M = 3.60s, SD = 1.11) than Precision-Stripe ($p$ \textless .001), Cursor-Sync (M = 4.32s, SD = 1.51, $p$ = .027), and One-Hand ($p$ \textless .001).
Moreover, Cursor-Sync has a faster completion time than the Precision-Stripe ($p$ = .033) and One-Hand ($p$ = .008).

There is a main effects on technique (F(4, 76) = 10.480, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .36).
Pairwise comparisons show that Simple-Ray (M = 4.07s, SD = 2.00) has a faster selection time than Precision-Stripe (M = 5.20s, SD = 2.48, $p$ = .004), Cursor-Sync (M = 4.71s, SD = 1.83, $p$ = .042), and One-Hand (M = 5.87s, SD = 2.58, $p$ \textless .001).
In addition, Simple-Stripe also results (M = 4.06s, SD = 2.11) faster than Precision-Stripe ($p$ = .009), Cursor-Sync ($p$ = .044), and One-Hand ($p$ \textless .001).
Moreover, Cursor-Sync is significantly faster than One-Hand ($p$ \textless .001).

A significant main effect is found on distance (F(1.552, 29.496) = 114.720, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .86).
Pairwise comparisons reveal that 3m (M = 3.71s, SD = 1.98) has a faster selection time than 6m (M = 4.41s, SD = 1.83, $p$ \textless .001) and 9m (M = 6.22s, SD = 2.34, $p$ \textless .001).
In addition, 6m is faster than 9m ($p$ \textless .001).
These results partially support \textbf{H1} and \textbf{H2}.




\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/error_distance_with_box.pdf}
% {ANOVA_Result_contents/figures/error_distance_with_box.pdf}
\caption{
Task 1 - Error Distance results with 95\% CI:
\dhk{Lower values indicate accurate performance, while
higher values are inaccurate. 
}
} 
\label{figure:ED_W/R}
\end{figure}

\subsubsection{Error Distance}

The results are reported in Figure \ref{figure:ED_W/R}.
A significant main effect is found on technique (F(4, 76) = 8.251, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .303).
Pairwise comparisons show that Simple-Ray has a smaller error distance (M = 22.26cm, SD = 6.77) than Simple-Stripe (M = 26.6cm, SD = 8.21, $p$ \textless .001), Cursor-Sync (M = 26.86cm, SD = 9.86, $p$ = .005), and One-Hand (M = 27.91cm, SD = 8.64, $p$ = .003).
In addition, Precision-Stripe has a significantly lower error distance (M = 20.35cm, SD = 7.32) than Simple-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ = .002).
These results do not support \textbf{H3} and \textbf{H4}.

% \subsubsection{Button Clicks}
% The results of the number of button clicks are reported in Figure \ref{figure:AT_W/R}. % and Table [].
% There is an interaction effect between technique and  distance (F(3.476, 66.041) = 16.239, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .461).
% Further analysis reveals that there are simple effects on technique at 6m (F(1.836, 34.879) = 4.563, $p$ = .020, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = 194) and 9m (F(2.465,46.831) = 23.826, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .556).
% Pairwise comparisons reveal that, at the 6m target position, Simple-Ray has more button clicks (M = 1.60, SD = 1.00) than Cursor-Sync (M = 1.03, SD = 0.11, $p$ = .012) and One-Hand Simultaneous (M = 1.03, SD = 0.11, $p$ = .020).
% In addition, Simple-Stripe leads to more button clicks (M = 1.50, SD = 0.63) than Cursor-Sync ($p$ = .001) and One-Hand Simultaneous ($p$ = .004).

% At 9m, Simple-Ray has more button clicks (M = 2.65, SD = 1.26) than Precision-Stripe (M = 1.58, SD = 0.82, $p$ = .002), Cursor-Sync (M = 1.08, SD = 0.34, $p$ < .001), and One-Hand Simultaneous (M = 1.00, SD = 0.00, $p$ < .001).
% In addition, Simple-Stripe (M = 3.10, SD = 1.35) has more button clicks than Precision-Stripe ($p$ = .002), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).

% There are main effects on technique (F(2.111, 40.113) = 18.430, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .492) and distance (F(1.403, 26.658) = 67.413, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .780).
% Pairwise comparisons show that Simple-Ray has more button clicks (M = 1.79, SD = 1.13) than Precision-Stripe (M = 1.28, SD = 0.60, $p$ = .011), Cursor-Sync (M = 1.05, SD = 0.24, $p$ \textless .001), and One-Hand Simultaneous (M = 1.04, SD = 0.21, $p$ \textless .001).
% In addition, Simple-Stripe (M = 1.89, SD = 1.23) has more button clicks than Precision-Stripe ($p$ = .002), Cursor-Sync ($p$ \textless .001), and One-Hand Simultaneous ($p$ \textless .001).
% Furthermore, Precision-Stripe has more attempts than Cursor-Sync ($p$ = .029) and One-Hand Simultaneous ($p$ = .008).

% Pairwise comparisons show that 3m (M = 1.08, SD = 0.27) has more button clicks than 6m (M = 1.28, SD = 0.62, $p$ \textless .001) and 9m (M = 1.88. SD = 1.24, $p$ < .001). In addition, 6m has more button clicks than 9m ($p$ \textless .001).


\subsubsection{NASA-TLX}

The NASA-TLX results are presented in the upper part of Table \ref{table:TLX_UEQ_W_B}.

\paragraph{Effort}
There is a main effect on Effort ($p$ = .016).
A pairwise comparison shows that Precision-Stripe has a lower effort rate than Simple-Stripe ($p$ = .014) and One-Hand ($p$ = .016).
In addition, Cursor-Sync has a lower Effort rate than Simple-Stripe ($p$ = .034) and One-Hand ($p$ = .018).

\paragraph{Frustration}
A main effect on Frustration ($p$ = .005) is found.
Pairwise comparisons reveal that Precision-Stripe has a lower value than Simple-Ray ($p$ = .006), Simple-Stripe ($p$ = .003), Cursor-Sync ($p$ = .016), and One-Hand ($p$ = .040).
In addition, Cursor-Sync has a lower Frustration rate than Simple-Ray ($p$ = .040).

There are no significant main effects on Mental Demand, Physical Demand, Performance, and Temporal Demand on technique.
\dhk{
These results are partially support our hypothesis (\textbf{H5}).
}

\subsubsection{UEQ}
The results of the UEQ are presented in the lower part of Table \ref{table:TLX_UEQ_W_B}.
\paragraph{Attractiveness}
There is a main effect on Attractiveness ($p$ = .043).
Pairwise comparisons show that Cursor-Sync has a higher value than Simple-Ray ($p$ = .021) and Simple-Stripe ($p$ = .047).

\paragraph{Efficiency}
There is a main effect on Efficiency ($p$ = .013).
Cursor-Sync has higher Efficiency rate than Simple-Stripe ($p$ = .037) and One-Hand ($p$ = .020).
In addition, Precision-Stripe has a higher Efficiency rate than One-Hand ($p$ = .036).

\paragraph{Dependability}
There is a main effect on Dependability ($p$ = .002). 
Comparisons show that Precision-Stripe has a higher Dependability rate than Simple-Ray ($p$ = .036) and One-Hand ($p$ = .023).
In addition, Cursor-Sync has a higher Dependability rate than Simple-Ray ($p$ = .005), Simple-Stirpe ($p$ = .032), and One-Hand ($p$ = .006).

There is no significant difference in Novelty, Perspicuity, and Stimulation among techniques.
These results are partially support our hypothesis (\textbf{H5}).

\subsection{Result: Task 2 \dhk{- \textit{without Reference}}}
\subsubsection{Selection Time}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/selection_time_without_box.pdf}
% {ANOVA_Result_contents/figures/response_time_without_box.pdf}
\caption{
% Task 2 - Selection Time result: Selection time results for each technique and distance (95\% CI error bar).
Task 2 - Selection Time results with 95\% CI.
\dhk{
Lower values indicate better/faster performance, whereas higher values signify poorer performance.
}
} 
\label{figure:RT_O/R}   
\end{figure}

The selection time results in Task 2 with each condition are reported in Figure \ref{figure:RT_O/R}.
These results show an interaction effect between the technique type and the target position distance (F(8, 152) = 13.324, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .412).
Further analysis reveals that there are simple effects on technique at 3m (F(1.944, 36.929) = 72.526, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .792), 6m (F(4, 76) = 49.594, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .723), and 9m (F(4, 76) = 59.515, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .758).
Pairwise comparisons reveal that, at the 3m target position, Simple-Ray has faster selection time (M = 1.71s, SD = 0.73) than Precision-Stripe (M = 2.90s, SD = 0.77, $p$ \textless .001), Cursor-Sync (M = 2.52s, SD = 0.73, $p$ \textless .001), and One-Hand (M = 5.05s, SD = 1.46, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 1.88s, SD = 0.60) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ \textless .001).
Furthermore, Precision-Stripe has a significantly faster selection than One-Hand ($p$ \textless .001).
Lastly, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .037) and One-Hand ($p$ \textless .001).

At 6m, Simple-Ray has faster selection time (M = 2.13s, SD = 1.06) than Precision-Stripe (M = 4.19s, SD = 1.39, $p$ \textless .001), Cursor-Sync (M = 3.47s, SD = 1.06, $p$ \textless .001), and One-Hand (M = 4.67s, SD = 1.39, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 2.35s, SD = 0.63) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ \textless .001).
Furthermore, Precision-Stripe has a significantly faster selection than One-Hand ($p$ = .037).
Lastly, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .014) and One-Hand ($p$ \textless .001).

At 9m, Simple-Ray has faster selection time (M = 2.41s, SD = 1.22) than Precision-Stripe (M = 5.22s, SD = 1.92, $p$ \textless .001), Cursor-Sync (M = 4.39s, SD = 1.37, $p$ \textless .001), and One-Hand (M = 5.44s, SD = 1.45, $p$ \textless .001).
In addition, Simple-Stripe leads to faster selection time (M = 2.60s, SD = 0.71) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ \textless .001).
Furthermore, Cursor-Sync has a faster selection time than Precision-Stripe ($p$ = .011) and One-Hand ($p$ \textless .001).

There are main effects on technique (F(4, 76) = 88.065, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .823) and distance (F(2, 38) = 56.226, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .747).

Pairwise comparisons show that Simple-Ray (M = 2.08s, SD = 1.05) has a faster selection time than Precision-Stripe (M = 4.11s, SD = 1.71, $p$ \textless .001), Cursor-Sync (M = 3.46s, SD = 1.31, $p$ \textless .001), and One-Hand (M = 5.05s, SD = 1.45, $p$ \textless .001).
In addition, Simple-Stripe has a faster result (M = 2.28s, SD = 0.71) than Precision-Stripe ($p$ \textless .001), Cursor-Sync ($p$ \textless .001), and One-Hand ($p$ \textless .001)
Furthermore, Simple-Stripe has a faster completion time than One-Hand ($p$ \textless .001), and Cursor-Sync has a faster completion time than Precision-Stripe ($p$ = .008) and One-Hand ($p$ \textless .001).

Pairwise comparisons show that 3m (M = 2.81s, SD = 1.50) is faster than 6m (M = 3.36s, SD = 1.50, $p$ \textless .001) and 9m (M = 4.01s, SD = 1.87, $p$ \textless .001).
In addition, 6m is faster than  9m ($p$ \textless .001).
These results support \textbf{H1} and \textbf{H2}.

\subsubsection{Error Distance}

\begin{figure}[t]
\centering
\includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/error_distance_without_box.pdf}
% {ANOVA_Result_contents/figures/error_distance_without_box.pdf}
\caption{
Task 2 - Error Distance results with 95\% CI:
\dhk{
Lower values indicate accurate performance, while
higher values are inaccurate. 
% Higher indicates worse performance (inaccurate) and lower indicates better performance (accurate).
}
} 
\label{figure:ED_O/R}   
\end{figure}


\begin{table*}[t]
\centering
% \caption{With-Reference task: selection time results with the technique and distance conditions}
\caption{Task 2 - NASA-TLX and UEQ results (Scales that have the main effect.)
The higher result indicates a worse result on mental demand and effort and a better result on performance, attractiveness, efficiency, perspicuity, dependability, and stimulation.
}
\begin{tabular} {m{2.2cm}| m{2.7cm}| m{0.7cm}| m{0.5cm} | m{1.4cm} | m{1.4cm}| m{1.4cm} | m{1.4cm}| m{1.4cm}}
\toprule 
    {\textbf{Mean (SD)}} & {\textbf{F}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}} & {\textbf{Simple-Ray}}  & {\textbf{Simple-Stripe}} & {\textbf{Precision-Stripe}} & {\textbf{Cursor-Sync}} & {\textbf{One-Hand}}\\ \midrule
% \begin{tabular} {m{2.2cm} | m{1.8cm} | m{2.0cm}| m{2.2cm} | m{1.8cm}| m{1.6cm}}
% \toprule 
    % {\textbf{Mean (SD)}} & {\textbf{Simple-Ray}}  & {\textbf{Simple-Stripe}} & {\textbf{Precision-Stripe}} & {\textbf{Cursor-Sync}} & {\textbf{One-Hand}}\\ \midrule
    % Interaction(T \texttimes D)  & {8, 152} & {7.247}  & {\textless .001} & {.276} \\ 
    % T  & {4, 76} &  {10.477}  & {\textless .001} & {.355} \\
    % D & {2, 38}  & {114.715} & {\textless .001} & {.858} \\
    Mental Demand & {F(3.07, 58.34) = 4.57} & {.006} & {.194} & {3.15 (1.66)} & {2.85 (1.79)} & {3.00 (1.69)} & {3.10 (1.97)} & {4.25 (1.94)}\\ 
    Performance & {F(4, 76) = 7.46} & {\textless .001} & {.282} & {4.85 (1.76)} & {4.95 (1.61)} & {5.35 (1.57)} & {4.80 (1.61)} & {3.65 (1.50)}\\
    Effort & {F(4, 76) = 5.15} & {\textless .001} & {.213} & {3.25 (1.89)} & {2.80 (1.40)} & {3.25 (1.80)} & {2.75 (1.68)} & {4.00 (1.89)}\\ \midrule
    Attractiveness & {F(2.39, 45.32) = 8.37} & {\textless .001} & {.306} & {1.18 (1.11)} & {1.14 (1.51)} & {1.58 (1.12)} & {1.31 (1.16)} & {0.18 (1.57)}\\ 
    Efficiency & {F(2.30, 43.79) = 5.42} & {.006} & {.222} & {1.59 (0.80)} & {1.58 (1.11)} & {1.75 (0.86)} & {1.81 (0.97)} & {0.79 (1.24)}\\ 
    Perspicuity & {F(2.49, 47.23) = 6.42} & {.002} & {.253} & {2.31 (0.81)} & {2.04 (1.28)} & {2.11 (1.02)} & {2.00 (1.23)} & {1.10 (1.32)}\\
    Dependability & {F(2.22, 42.17) = 6.89} & {.002} & {.266} & {1.09 (0.94)} & {1.24 (0.88)} & {1.39 (0.84)} & {1.33 (0.97)} & {0.37 (1.21)}\\
    Stimulation & {F(4, 76) = 4.26} & {.004} & {.183} & {0.86 (1.23)} & {0.88 (1.48)} & {1.21 (1.19)} & {1.20 (0.97)} & {0.23 (1.34)}\\
    \bottomrule
\end{tabular}
\label{table:TLX_UEQ_Without_B}
%\vspace{-0.6cm}
\end{table*}

The error distance results with each condition are reported in Figure \ref{figure:ED_O/R}.
There is an interaction effect between technique and target position distance (F(8, 152) = 11.634, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .380).
Further examination shows significant simple effects of the techniques at distances of 3m (F(2.505, 47.596) = 24.371, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .562), 6m (F(4, 76) = 12.079, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .389), and 7m (F(1.755, 33.350) = 9.300, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .329).



Pairwise comparisons show that, with a 3m located target, One-Hand (M = 50.60cm, SD = 21.37, $p$ \textless .001) has significantly lower accurate rates than Simple-Ray (M = 22.50cm, SD = 14.30), Simple-Stripe (M = 17.61cm, SD = 9.25),  Precision-Stripe (M = 18.80cm, SD = 14.69) and Cursor-Sync (M = 14.83cm, SD = 7.37).
In addition, Simple-Ray is less accurate than the Cursor-Sync ($p$ = .041) technique.

With a 6m condition,  Simple-Stripe has more accurate results (M = 51.68cm, SD = 23.42) than Simple-Ray (M = 70.58cm, SD = 40.13, $p$ = .025) and One-Hand (M = 91.70cm, SD = 49.75, $p$ = .001).
Precision-Stripe is also more accurate (M = 42.04cm, SD = 34.58) than Simple-Ray ($p$ = .002) and One-Hand ($p$ \textless .001). 
Moreover, Cursor-Sync is more accurate (M = 32.72cm, SD = 19.74) than Simple-Ray ($p$ \textless .001), Simple-Stripe ($p$ = .014), and One-Hand ($p$ \textless .001) techniques.

With a 9m condition, Simple-Ray is less accurate (M = 161.01cm, SD = 117.66) than Precision-Stripe (M = 77.78cm, SD = 32.08, $p$ = .002), Cursor-Sync (M = 66.33cm, SD = 35.23, $p$ \textless .001), and One-Hand (M = 71.42cm, SD = 32.26, $p$ = .006).
Simple-Stripe technique is also less accurate (M = 114.71cm, SD = 45.74) than Precision-Stripe ($p$ = .013), Cursor-Sync ($p$ = .003), and One-Hand ($p$ = .001).

There are main effects on technique (F(4, 76) = 9.294, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .328) and distance (F(2, 38) = 90.853, $p$ \textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$} = .827). 
Pairwise comparisons show that Precision-Stripe has a less error distance (M = 46.21cm, SD = 37.21) than Simple-Ray (M = 84.70cm, SD = 91.63, $p$ \textless .001) and One-Hand (M = 71.24cm, SD = 39.57, $p$ = .002).
In addition, Cursor-Sync has a less error distance (M = 37.96cm, SD = 31.72) than Simple-Ray ($p$ \textless .001), Simple-Stripe (M = 61.34cm, SD = 50.23, $p$ = .004), Precision-Stripe ($p$ = .046), and One-Hand ($p$ \textless .001).
Lastly, the participants complete the task more accurately when a target position is 3m (M = 24.87cm, SD = 19.20) than 6m (M = 57.74cm, SD = 40.54, $p$ \textless .001) and 9m (M = 98.25cm, SD = 70.57, $p$ \textless .001), and also, the result from 6m is more accurate than from 9m ($p$ \textless .001).
\dhk{
These results partially support \textbf{H3} and \textbf{H4}.
}
\subsubsection{NASA-TLX}

% \begin{figure}[t]
% \centering
% \includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/TLX_without_box.pdf}
% % {ANOVA_Result_contents/figures/TLX_without_box.pdf}
% \caption{
% Task 2 - NASA-TLX result (95\% CI error bar):
% \dhk{
% Higher indicates worse and lower indicates better workload for mental demand and effort.
% In contrast, for performance, higher indicates better, and lower indicates worse.
% }
% } 
% \label{figure:TLX_O/R}   
% \end{figure}

The NASA-TLX results are shown in the upper part of the Table \ref{table:TLX_UEQ_Without_B}.

\paragraph{Mental Demand}
There is a main effect on Mental Demand ($p$ = .006).
Pairwise comparisons show that One-Hand has a higher Mental Demand rate than Simple-Ray ($p$ = .005), Simple-Stripe ($p$ = .001), Precision-Stripe ($p$ = .008), and Cursor-Sync ($p$ = .012).

\paragraph{Performance}
 In addition, there is a significant main effect on Performance ($p$ \textless .001).
 One-Hand has lower performance rate than Simple-Ray ($p$ \textless .001), Simple-Stripe ($p$ \textless .001), Precision-Stripe ($p$ \textless .001), and Cursor-Sync ($p$ \textless .001).

\paragraph{Effort}
There is a main effect on Effort ($p$ \textless .001).
One-Hand has higher Effort rate than Simple-Ray ($p$ = .021), Simple-Stripe ($p$ = .006), and Cursor-Sync ($p$ = .002).
However, there is no difference between One-Hand and Precision-Stripe, and among Simple-Ray, Simple-Stripe, and Cursor-Sync.

There is no significant main effect on Frustration, Physical Demand, and Temporal Demand.
\dhk{
These results are partially support our hypothesis (\textbf{H5}).
}
\subsubsection{UEQ}

% \begin{figure}[t]
% \centering
% \includegraphics[angle=270, width=.45\textwidth]{ANOVA_Result_contents/figures/tight/UEQ_without_box.pdf}
% % {ANOVA_Result_contents/figures/UEQ_without_box.pdf}
% \caption{
% Task 2 - UEQ result (95\% CI error bar):
% \dhk{
% Higher indicates better experience and lower indicates worse experience.
% }
% } 
% \label{figure:UEQ_O/R}   
% \end{figure}

The UEQ results are presented in the bottom part of the Table \ref{table:TLX_UEQ_Without_B}.

\paragraph{Attractiveness}
There is a main effect on Attractiveness ($p$ \textless .001).
Pairwise comparisons show that One-Hand has a lower Attractiveness rate than Simple-Ray ($p$ \textless .001), Simple-Stripe ($p$ = .012), Precision-Stripe ($p$ \textless .001), and Cursor-Sync ($p$ = .003 ).
In addition, Simple-Stripe has a lower Attractiveness rate than Precision-Stripe ($p$ = .022).

\paragraph{Efficiency}
There is a main effect on Efficiency ($p$ = .006).
One-Hand has a lower Efficiency rate than Simple-Ray ($p$ = .011), Simple-Stripe ($p$ = .039), Precision-Stripe ($p$ = .005), and Cursor-Sync ($p$ = .008).

\paragraph{Perspicuity}
There is a main effect on Perspicuity ($p$ = .002).
One-Hand has a lower perspicuity rate than Simple-Ray ($p$ \textless .001),  Simple-Stripe ($p$ = .007), Precision-Stripe ($p$ = .002), and Cursor-Sync ($p$ = .026).

\paragraph{Dependability}
Moreover, there is a main effect on Dependability ($p$ = .002).
One-Hand has a lower Dependability rate than Simple-Ray ($p$ = .029), Simple-Stripe ($p$ = .005), Precision-Stripe ($p$ = .002), and Cursor-Sync ($p$ = .006). 

\paragraph{Stimulation}
Lastly, there is a main effect on Stimulation ($p$ = .004).
One-Hand has a lower Stimulation rate than Simple-Ray ($p$ = .020), Precision-Stripe ($p$ = .011) and Cursor-Sync ($p$ = .006).
However, there is no significant difference between One-Hand and Simple-Stripe.

The Novelty of each technique is not significantly different in this task.
\dhk{
These results are partially support our hypothesis (\textbf{H5}).
}

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> contents/0_introduction.tex <==
\section{Introduction}

Selection represents a core interaction within immersive virtual environments (IVE), playing a crucial role in both object manipulation and the facilitation of several navigation techniques. These navigation techniques enable users to traverse the IVE space, requiring the selection or specification of a target location ~\cite{argelaguet2013survey}.
For example, Teleportation~\cite{prithul2021teleportation} allows users to move to a desired position immediately, but the user must select a target position.
Importantly, the scope of navigation is not confined to ground level, allowing for a comprehensive spatial interaction that encompasses various elevations and dimensions \cite{weissker2023gaining}.
However, these techniques are required to select a tangible object in IVE, such as a ground or a virtual object to move close to, to engage with the navigation, which would limit the selected area for those navigation techniques. 

Mid-air selection can be defined as a technique that enables the user to point and select an intangible object within a 3D space.
Previous studies have utilized scene-in-hand metaphor \cite{ware1990exploration} along with arm-extension techniques \cite{li2018evaluation, cho2015evaluation}, a parabolic ray starting from a ground position, or combining keys to control different degrees of freedom (DOF) \cite{weissker2023gaining} to facilitate mid-air selection.
Nonetheless, these approaches have restrictions such as constraints being on the ground, a limited range of selections and inaccurate position selection due to the sensitivity of the offset gain factors \cite{li2018evaluation}.

In this paper, we introduce bimanual mid-air selection techniques that can address these issues, allowing users to intuitively and accurately select mid-air positions in IVE where they can see.
Our bimanual mid-air selection techniques work by using two linear rays emanating from both hands to create an intersection point and using the point as a selecting position. On top of this Simple-Ray technique, a visual aid and selection mechanisms are added to enhance the selection accuracy and user experience.
Simple-Stripe has 1-meter length stripes on a ray. Precision-Stripe allows the user to select one of the 1-meter length stripes and making the intersection point only be located within the selected 1 meter.
Cursor-Sync allows the user to create an intersection point inside the stripe located closest to the controller.  

We evaluate the performance of these techniques in two types of mid-air selection tasks with 20 participants.
The first mid-air selection task asks to select a mid-air position near an object located to evaluate the performance of selecting a given mid-air position.
The second selection task asks to select a mid-air position where a target object was located for 1.5 seconcds.
This task evaluates the performance of selecting a mid-air position that a user wants to select.
Both tasks are conducted at close (3m), middle (6m), and far (9m) distances to investigate how performance varies by distance.
The results show that the Simple-Ray allows a user to select a position quickly.
Unexpectedly, the Simple-Stripe represents a not different selecting time and accurate results both from the Simple-Ray results.
The Precision-Stripe has relatively better accuracy at meddle and far distances, but the selection time is the slowest among the evaluated bimanual techniques.
Interestingly, the Cursor-Sync technique allows a user to select a mid-air position significantly faster than the Precision-Stripe, but different from the expectation, the accuracy is not significantly different.
The One-hand Simultaneous mid-air technique~\cite{weissker2023gaining} that is evaluated for comparison generally shows inaccurate selections and late selection than the bimanual techniques.
As a result, we propose the concept of the bimanual mid-air selection technique and its variations for efficient mid-air navigation, and we hope that a user can have a better mid-air navigation experience in various VR environments through these techniques. The main contributions of this paper are the following:

\begin{itemize}
\item{
We introduce bimanual mid-air selection techniques with visual aids and support features to improve the selection technique in IVE.
These techniques are implemented as two straight rays, with the intersection point between the rays functioning as a cursor for selecting a mid-air location.
}

\item{
We present the disparity in performance among each mid-air technique and also investigate user experiences.
We evaluated our techniques with 20 participants, and the results demonstrate the pros and cons of each technique under various task and distance conditions.}
\end{itemize}

==> contents/1_related_works.tex <==
\section{Related Works}
%Selection?
\subsection{Mid-Air Selection}
\paragraph{Direct Selection}
Direct selection with a controller is the primary method for selecting objects in VR, similar to grabbing objects in your hand in the real world~\cite{jacoby1994gestural,mine1997moving}.
It allows users to perform mid-air selection within their arm's reach space.
However, it has a limitation of selecting distant coordinates beyond their arm reach~\cite{song1993nonlinear}.
To address such a limitation, selection techniques for distant objects have been developed, some of which can be adaptable to mid-air selection.
An example of such a method is the arm extension metaphor, including Go-Go and the linear offset technique~\cite{poupyrev1996go,li2015evaluation}.
\dhk{} % SImilar cases with Go-Go
These techniques entail the mapping of virtual cursors or hands exponentially or with a designated offset, contingent on the distance between the user and the controllers.
It enables virtual cursors to extend beyond the actual controller position.
However, if increase the arm extension ratio to select far away, it decreases selection performance, such as selection time and accuracy~\cite{li2015evaluation}.
% Change the world Size
\dhk{
Another approach to solving arm reach limitation is decreasing the size of the world~\cite{pausch1995navigation,stoakley1995virtual, bell2001view}.
With this method, a user can directly select a position, even a mid-air position, from a different viewpoint, as if looking down from the sky.
Also, this method not only extends the selectable area but also presents the occluded position behind objects.
However, the different scale viewpoints can make selecting a position hard for a user, and when the scale ratio is changed, the difficulty can be increased~\cite{wingrave2006overcoming}.
}

\paragraph{Ray Selection}
Next, the ray casting metaphor, in which rays emerge from controllers, eyes, or the head, is a popular method for remote object selection.
Diverse ray casting techniques have been introduced to achieve accurate and fast distant object selection in a variety of scenarios.
For example, Lu et al.~\cite{lu2020investigating} introduced 3D Bubble Cursor, which uses a heuristic approach to provide a sphere cursor that dynamically adjusts its size to always capture the closest target from the ray.
Steinicke et al.~\cite{steinicke2006object} presented the Sticky-Ray selection technique, which is based on a bendable ray that points to the closest selectable object.
However, many of these variations still require target objects and do not support mid-air selection as they only take into account 2 DOF of pitch and yaw controller rotation for remote object selection.
A way to make the ray casting technique enable mid-air selection is additional degrees of freedom to control the depth of the ray by a ray that has been manipulated using multimodal input.
Previous research incorporated depth control into the ray casting metaphor to address remote object selection issue in occlusion. 
Baloup et al. introduced RayCursor~\cite{baloup2019raycursor}, allowing depth adjustment of ray selection by adding a cursor that can move forward and backward using controller buttons.
Ro et al.\cite{ro2017dynamic} proposed a similar approach using a smartphone.
Similarly, Zhai et al.~\cite{zhai1996partial} presented Silk Cursor, a 3D volume cursor rather than a 3D point cursor.
% Curved Ray
\dhk{
A ray can also select a mid-air position by changing the height of a cutoff layer.
Parabola teleportation is the most common teleportation method that selects a position on the ground using a curved ray~\cite{funk2019assessing}.
In that case, the curved ray is cut at the ground level to select a position on the ground, but when the height of the cutoff layer is changed, this curved ray can now select the mid-air position.
~\cite{weissker2023gaining}.
}

\subsection{Bimanual Selection}
Another multimodal approach is using two hands.
Using a bimanual technique on a single task can provide better performance than the usage of an unimanual technique~\cite{buxton1986study}.
Owen et al.~\cite{owen2005gets} suggested design principles to better bimanual technique than unimanual: visually integrated, conceptually integrated, and integrated device spaces.
And this improvement is more effective when a task gets more difficult.

Several studies tried to improve the unimanual technique using the bimanual approach.
Ulinski et al.~\cite{ulinski2007two,ulinski2009selection} had a volumetric data interaction study focused on the technique's symmetricity.
Their study suggested a design principle for the bimanual selection technique: a symmetric technique can increase selection speed, and an asymmetric structure can decrease fatigue.
Chaconas et al.~\cite{chaconas2018evaluation} investigated a bimanual manipulation technique in an augmented reality environment.
Their technique can have rotation and scale operations using a bimanual gesture system without controllers, and its user study results indicate that the bimanual technique can have a place in the future of augmented reality.

The bimanual technique can also even increase the number of DOF~\cite{cho2015evaluation,feng2015comparison,li2015evaluation}.
While a user controls the two 6 DOF controllers, the relative position between the controllers allows them to handle the additional DOF, resulting in a consequent 7 DOF system.
The additional DOF was used to control the scale of a selected object intuitively in the studies, but it still has the potential to be used as various features, such as tension control.

The bimanual approach also applies on the ray casting based technique.
This approach addresses the limitations of unimanual ray casting by distinguishing between quick but rough and fine selection tasks.
The fine selection activity gives users control over the depth of ray selection, resulting in mid-air selection.
Wyss et al.~\cite{wyss2006isith} and Zhang et al.~\cite{zhang2022conductor} introduced bimanual ray casting techniques called iSith and Conductor, respectively.
iSith is a intersection-based selection technique that employs two rays emerging from both hands, whereas Conductor uses one ray for the dominant hand and a rectangle-like wide ray for the minor hand.
Zhang et al. conducted a user study and found Conductor outperformed RayCursor in remote target selection, but did not compare its performance to iSith.
Chen et al.~\cite{chen2023gazeraycursor} introduced the GazeRayCursor, a multimodal ray control approach that uses both eyes and controllers.

Although previous intersection-based bimanual studies did not investigate mid-air selection, these bimanual selection techniques have the potential to intuitively and effectively select a mid-air position.
In this paper, we investigate the intersection-based bimanual technique for mid-air selection.
Additionally, using the distance conditions (near, medium, and far away), we investigate the potential use of it as mid-air navigation's destination selection technique.

\cite{bowman1999testbed}
\cite{bowman1997evaluation}
\cite{feiner2003flexible}
\cite{hinckley1994survey}

==> contents/2_techniques.tex <==
% \section{Crossing Rays, Mid-Air Selection Technique}
\section{Crossing Rays for Mid-Air Selection}
This section introduces our bimanual mid-air selection technique, Crossing Rays, along with its variants designed to enhance the selection accuracy and user experience.
 A recognized challenge with ray-based selection techniques is the difficulty encountered when the target is situated at a distance, which is known as the Heisenberg effect \cite{wolf2020understanding}.  This issue persists in the context of mid-air selections, affecting the precision and ease of target acquisition from afar. To tackle this challenge, we designed and developed three ray-based selection variants -- namely \textbf{Simple-Stripe}, \textbf{Precision-Stripe}, and \textbf{Cursor-Sync} --  alongside the basic \textbf{Simple-Ray} selection technique, to improve the accuracy of mid-air selections. Furthermore, we detail the \textbf{One-Hand Simultaneous} selection technique introduced by Weissker et al. \cite{weissker2023gaining} as a technique utilized in our user study to assess the efficiency and usability of our techniques.

\subsection{Basic Crossing Ray Technique: Simple-Ray}
The Crossing Ray technique allows mid-air selection by intersecting two straight rays projected from the controllers held in each hand, a mechanism introduced by Wyss et al. \cite{wyss2006isith}. By default, it shows two simple white rays. Users can control the intersection point by altering the orientation of the controllers, directing them inward or outward. Additionally, they can adjust the intersection point by moving the controllers either closer to or farther.
In accordance with Guiard's framework \cite{guiard1987asymmetric}, the ray emitted from the dominant hand targets the desired point, while the ray from the non-dominant hand establishes a reference frame for the dominant hand, facilitating coordinated action and spatial orientation. 

When two rays are interested, a sphere cursor is visible as shown in Figure~\ref{figure:techniques}A. The cursor is 0.1m radius white sphere. The cursor appears when the two rays are less than 0.2m apart orthogonally, even if they do not intersect perfectly. This design choice aims to minimize user's arm fatigue and simplify the technique's utilization. 

\begin{figure*}[t]
\centering
\includegraphics[angle=0, width=.95\textwidth]{figures/Techniques_v3.pdf}
\caption{
Technique variations:
A) \textbf{Simple-Ray}: Two rays from each controller make an intersection point, pointing to a mid-air position.
B) \textbf{Simple-Stripe}: The base is the Simple-Ray technique, and 1-meter length stripes are on the ray of the dominant hand side.
C) \textbf{Precision-Stripe}: The intersection point can only be located in the selected range, one of the stripes.
D) \textbf{Cursor-Sync}: The selecting point's relative position in the selected range is synchronized with the position of the intersection point in the closest stripe.
E) \textbf{One-Hand Simultaneous}: The unimanual mid-air selection with parabolic ray, which can control vertical position using a joystick on the controller pushing (upward) and pulling (downward).
} 
\label{figure:techniques}   
\end{figure*}


\subsection{Simple-Stripe}
It presents a visual aid of alternating black and white stripes along the ray projected from the controller in the dominant hand, as shown in Figure~\ref{figure:techniques}B.
Each black or white stripe measures 1m.
By integrating stripes to function as a visual ruler, this technique is expected to enhance the user's ability to perceive depth and accurately determine mid-air position within the virtual space. The incorporation of these stripes into the ray selection process introduces a novel layer of user interaction by providing a clear, measurable reference for assessing spatial information in the virtual environment.

\subsection{Precision-Stripe}
This technique builds upon the Simple-Stripe technique by incorporating an extra step where a stripe is selected prior to the final mid-air selection. This modification enables users to confine the scope of mid-air selection, thereby minimizing the likelihood of unintended cursor movements—either further away or closer—due to fluctuations in the controller's position  (Figure~\ref{figure:techniques}C. This feature could be particularly beneficial when the target is positioned at a distance from the users. Selection of a stripe is facilitated through the joystick of the dominant hand's controller.

\subsection{Cursor-Sync}
Cursor-Sync empowers users to maneuver the cursor within the first stripe of the dominant ray proximal to them, as illustrated in Figure~\ref{figure:techniques}D.
Initially, upon selecting a stripe of interest, two cursors materialize. One within the chosen stripe and another in the first stripe of the dominant ray. The positions of these cursors within their respective stripes are synchronized.
Subsequently, when users adjust the position of the near-cursor using the non-dominant ray, the cursor within the selected range of interest correspondingly shifts.
With this technique, users could precisely control the selection point, enhancing accuracy and interaction efficiency within the virtual environment.

\subsection{One-Hand Simultaneous}
Weissker et al. introduced the One-Hand Simultaneous technique for mid-air teleportation \cite{weissker2023gaining}.
Users can utilize the One-Hand Simultaneous technique through a touchpad to adjust their target position vertically while concurrently moving the controller to pinpoint the desired location. Their research highlights the advantages of the One-Hand Simultaneous teleportation technique compared to the other two methods. The Two-Step technique enables users to choose a target location at the same elevation and adjust the controller's tilt to move vertically.
Conversely, the Separate technique requires users to modify the elevation first, followed by teleportation within that same elevation level.
The findings indicate that the simultaneous technique achieves the highest accuracy, despite resulting in longer specification times and increased task load compared to the other two techniques. Due to its straightforward control mechanism and higher accuracy for mid-air selection, we employed this technique as a base condition to evaluate our techniques. 

In our study, we implemented the One-Hand Simultaneous technique utilizing a parabolic ray with a cursor at its end (Figure~\ref{figure:techniques}E.


==> contents/3_experiment.tex <==

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.47\textwidth]{figures/Experiment_v4.pdf}
\caption{
A) Experiment room: 15m width, depth, and height empty experiment room with a 5m height pillar for a participant.
B) Target position: The target position is located in front of the participant with three difference distance conditions (3m, 6m, and 9m). The location is 10 degrees away from the central axis.
C) Task 1: The target position is 50cm in front of a reference object(Wooden box). The participant can only select within 50cm of the target position.
D) Task 2: A red sphere is 1.5 seconds showing on a target position. While the red sphere is shown, the participant could not make the intersection point, or control an aim sphere from the One-Hand Simultaneous technique. But, when the technique condition is bimanual, the dominant hand side ray is provided.
} 
\label{figure:experiments}   
\end{figure}

\section{Experiment design}
In this section, we outline the design of our user study aimed at assessing the usability and efficiency of the mid-air selection techniques described in Section 3.

\subsection{Experiment Tasks}
For the study, we crafted two mid-air selection tasks to accommodate two distinct scenarios within a VR environment. The initial scenario involves selecting a mid-air position adjacent to a virtual object, whereas the subsequent scenario entails choosing a mid-air position in the absence of reference objects.

\subsubsection{Task 1: Mid-Air Selection with Reference} 
This task involves selecting a position located 0.5 meters in front of a reference object suspended in mid-air. The reference object, a wooden box, is oriented such that its facing side is perpendicular to the user (Figure~\ref{figure:experiments}C). 
The target position varies across three different distance conditions (3m, 6m, and 9m) and is positioned 10 degrees away from the central axis.
Participants are required to use a specific selection technique to identify the target position. Selections are only valid if made from a minimum distance of 50 centimeters away from the target location.  Participants click a button and the position does not align with this threshold, they must click again until the selection criteria are met. 

In this task, the presence of a reference object eliminates the need for participants to remember the mid-air position, allowing them to concentrate solely on selecting the designated location.
The measurement focuses on the selection time required for a participant to accurately select the correct position over multiple attempts. Therefore, the selection time reflects the participants' ability to quickly identify a strictly designated object or position. Meanwhile, the selection accuracy serves as an indicator of how effectively a technique assists users in gauging distance from a nearby object.

\subsubsection{Task 2: Mid-Air Selection without Reference}
 This task requires selecting a mid-air position previously occupied by a red sphere.
The red-sphere is at one of three distinct distance conditions (3m, 6m, and 9m) and offset by 10 degrees from the center.
The sphere is displayed for 1.5 seconds at the start of the task, after which participants are required to recall and select the sphere's position once it has disappeared. 

During the red-sphere is visible, only one ray from the dominant hand is visible for the crossing rays techniques, whereas no ray is visible with the one-hand simultaneous technique.
In contrast to Task 1, the absence of a reference object necessitates that users remember the designated position, challenging them to select based on memory, which can be viewed as a measure of intentional position selection.

This setup evaluates each technique's effectiveness in facilitating a user's ability to intentionally select a mid-air position.
Selection accuracy measures how well a technique assists in perceiving and remembering a target position. 

\subsection{Measurement}

For Task 1, three quantitative metrics are recorded to assess user performance: selection time, error distance, and the number of button clicks. Selection time measures how quickly the participant performs the selection task without a reference object.  Error distance calculates the discrepancy between the target position and the participant's selected position.
The number of button clicks is measured by how many times a participant clicks a button to select the target position within a specified threshold (i.e., 50 cm.)
In Task 2, selection time and error distance are the primary metrics of interest, as participants are required to select a target position only once. 

Following each technique and task, participants complete two questionnaires: the NASA-TLX, which assesses 6 categories (Mental Workload,
Physical Workload, Temporal Load Operation, Performance Capability, Effort, and Sense of Frustration) as detailed by \cite{hart1988development,hart2006nasa}, and the User Experience Questionnaire (UEQ) for evaluating 6 different aspects of user experience including (Attractiveness, Perspicuity,
Efficiency, Dependability, Stimulation, and Novelty) as outlined by \cite{laugwitz2008construction}. These instruments gauge the participants' VR experiences with the respective technique and task.

\subsection{Procedure}
When a participant arrives at a study location, he or she is asked to read and sign a consent form according to the IRB protocol (\#13746).
The participant then completes a demographic questionnaire about their age and VR experience.
Following that, the participant is briefed on the experiment's purpose, procedure, and tasks.
The participant practiced each technique and selection task right before the experiment with that technique and task type condition.
Each participant performs a total of 180 selection tasks (5 techniques \texttimes{} 2 tasks \texttimes{} 3 distances \texttimes{} 6 times repeat).
The technique order is counterbalanced across all participants, while the distance is randomly ordered for the tasks.
After completing a task using a given technique under a task type, the participant is asked to complete the NASA-TLX and UEQ questionnaires.

\subsection{Hypothesis}
We set the following five hypotheses based on the designed experience and techniques to find answers to the research questions.

\begin{itemize}
\item[\textbf{H1}] Simple-Ray and Simple-Stripe are expected to have faster selection time than other mid-air selection techniques as they do not incorporate an additional clutch that could potentially delay selection.

\item[\textbf{H2}] Cursor-Sync is expected to have a faster selection time than Precision-Stripe and One-hand Simultaneous because it supports features for precise selection and decreases the time spent on detail control.

\item[\textbf{H3}] Precision-Stripe and Cursor-Sync are expected to have higher accuracy compared to other mid-air selection techniques due to visual aids and support features that facilitate precise selection. 

\item[\textbf{H4}] Simple-Stripe is expected to have higher accuracy than Simple-Ray and One-Handed Simultaneous due to visual aid.

\item[\textbf{H5}] Simple-Stripe, Precision-Stripe and Cursor-Sync are expected to provide better usability and less workload than Simple-Ray and One-Handed Simultaneous because of the visual aid and support feature.

\end{itemize}

\subsection{Participants}
A total of 20 participants (7 males and 13 females) are recruited from the university's participant recruitment system (SONA).
The minimum participant number to ensure the statistical effect size is 16. 
The number is calculated using the G*power analysis tool\cite{faul2007g} with the following parameters: effect size = 0.4, alpha = 0.05, and power = 0.9.
Their average age is 19.3, with a range of 18 to 22 years. All participants have 20/20 (or corrected 20/20) vision, and they do not have physical impairments in using VR devices.
They were rewarded 2 SONA credits as follows the university SONA policy. According to the pre-questionnaire, 13 out of 20 participants have VR experience. 
\subsection{Apparatus}
The Meta Quest 3 and its two controllers are utilized.
It features a 110$^\circ$ horizontal and 96$^\circ$ vertical Field of View (FoV), and its resolution is 2064 \texttimes{} 2208 pixels per eye.

We present the target position located within 60$^\circ$ FoV in all conditions.
The experiment application is developed by Unity 2022.3.3f1 and runs on a Windows 10 desktop with an Intel Xeon W-2245 CPU(3.90GHz), 64GB RAM, and Nvidia GeForce RTX 3090 graphics card.

==> contents/4_1_result_boots_task_1.tex <==
\section{Result}
\subsection{Task 1: With Reference Object}
\subsubsection{Selection Time}


\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.5\textwidth]{figures/selection_time_withB.pdf}
\caption{
Task 1 - Selection Time: Selection time results for each technique and each distance condition.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:ST_withB}   
\end{figure}

A summary of the selection time results for each technique and distance conditions in Task 1 is illustrated in Fig \ref{figure:ST_withB}.
The mean Selection time results for each technique are: Simple-Ray = 4.066s $_{[3.627, 4.669]}$, Simple-Stripe = 4.059s $_{[3.589, 4.645]}$, Precision = 5.199s $_{[4.663, 5.936]}$, Sync = 4.711s $_{[4.269, 5.200]}$, and OneHand = 5.865s $_{[5.285, 6.615]}$.
The results for each distance condition to the target are: 3m = 3.712s $_{[3.364, 4.149]}$, 6m = 4.410s $_{[4.095, 4.830]}$, and 9m = 6.219s $_{[5.807, 6.726]}$.

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.5\textwidth]{figures/diff_task_1_selection_time_withB.pdf}
\caption{
Task 1 - Selection Time Comparison: Selection time result comparisons between each technique and each distance condition.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:diff_ST_withB}   
\end{figure}

A summary of the selection time comparison results between technique conditions and between target distance conditions in Task 1 is illustrated in Fig \ref{figure:diff_ST_withB}.
From this selection time results, using the Simple-Ray technique is 1.145s $_{[1.037, 1.267]}$ faster than Precision, 0.629s $_{[0.555, 0.681]}$ faster than Sync, and 1.801s $_{[1.659, 1.947]}$ faster than OneHand techniques.
Due to the using Simple-Ray is just 0.023s $_{[0.0064, 0.0377]}$ faster than using Simple-Stripe, the comparisons between using Simple-Stripe and others are similar.
Using the Simple-Stripe technique is 1.168s $_{[1.074, 1.291]}$ faster than Precision, 0.629s $_{[0.555, 0.681]}$ faster than Sync, and 1.824s $_{[1.697, 1.971]}$ faster than OneHand techniques.
Using the Precision technique is 0.539s $_{[0.394, 0.736]}$ slower than Sync, but 0.659s $_{[0.622, 0.680]}$ faster than OneHand technique.
And lastly, using the Sync technique is 1.195s $_{[1.016, 1.415]}$ faster than OneHand technique.

The distance to the target position also affects the selection time.
When the target position is 3m, the selection is 0.733s $_{[0.687, 0.731]}$ faster than at 6m and 2.509s $_{[2.465, 2.577]}$ faster than at 9m.
Likewise, the target at 6m is selected 1.806s $_{[1.713, 1.896]}$ faster than the target at 9m.


\subsubsection{Error Distance}

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.5\textwidth]{figures/error_distance_withB.pdf}
\caption{
Task 1 - Error Distance: Error distance result for each technique and each distance condition.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:ED_withB}   
\end{figure}

A summary of the error distance results for each technique and distance conditions in Task 1 is illustrated in Fig \ref{figure:ED_withB}.

The error distance results are different depending on the technique used.
The mean Error distance results for using each technique are: Simple-Ray = 22.26cm $_{[20.67, 24.04]}$, Simple-Stripe = 26.58cm $_{[24.54, 28.69]}$, Precision = 20.35cm $_{[18.55, 22.29]}$, Sync = 26.86cm $_{[24.37, 29.28]}$, and OneHand = 27.91cm $_{[25.63, 30.10]}$.
The results for each distance condition to the target are: 3m = 23.53cm $_{[21.86, 25.30]}$, 6m = 24.95cm $_{[23.33, 26.54]}$, and 9m = 25.89cm $_{[24.16, 27.72]}$.

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.5\textwidth]{figures/diff_task_1_error_distance_withB.pdf}
\caption{
Task 1 - Error Distance Comparison: Error Distance result comparisons between each technique and each distance condition.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:diff_ED_withB}   
\end{figure}

A summary of the error distance comparison results between techniques and between target distance conditions in Task 1 is illustrated in Fig \ref{figure:diff_ED_withB}.
Consequently, comparisons between results with using each technique are as follows: error distance by Simple-Ray technique is 4.284cm $_{[3.877, 4.657]}$ smaller than by Simple-Stripe, 4.516cm $_{[3.702, 5.245]}$ smaller than by Sync, and 5.563cm $_{[4.969, 6.065]}$ smaller than by OneHand techniques, but 1.924cm $_{[1.747, 2.114]}$ larger than by Precision technique.
Similarly, the error distance result from the Simple-Stripe technique is 1.279cm $_{[1.092, 1.408]}$ smaller than that from the OneHand technique but 6.208cm $_{[5.991, 6.403]}$ larger than that from the Precision technique.
Comparisons between rest combinations show that the error distance result from the Precision technique is 6.440cm $_{[5.816, 6.992]}$ smaller than that from Sync and 7.487cm $_{[7.083,7.812]}$ smaller than that from the OneHand technique.
Also, the Sync technique's result is 1.047cm $_{[0.820, 1.267]}$ smaller than that of the OneHand technique.

Results between distance conditions show that when the target is at 3m, the error distance is 1.374cm $_{[1.240, 1.465]}$ smaller than at 6m and 2.358cm $_{[2.319, 2.417]}$ smaller than at 9m.
Also, the result at 6m is 0.983cm $_{[0.869, 1.177]}$ smaller than at 9m.

\subsubsection{NASA TLX}

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.45\textwidth]{figures/TLX_result_withB_TLX.pdf}
\caption{
Task 1 - NASA TLX. 
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:TLX_withB}   
\end{figure}

A summary of the NASA-TLX qualitative results are illustrated in Fig \ref{figure:TLX_withB}.
The mental demand dimension results for each technique are: Simple-Ray = 3.300 $_{[2.550, 4.100]}$, Simple-Stripe = 3.300 $_{[2.450, 4.200]}$, Precision = 2.550 $_{[1.900, 3.300]}$,Sync = 2.700 $_{[2.000, 3.550]}$, and OneHand = 3.650 $_{[2.800, 4.400]}$.
The physical demand dimension results for each technique are: Simple-Ray = 2.050 $_{[1.550, 2.600]}$, Simple-Stripe = 2.000 $_{[1.450, 2.850]}$, Precision = 1.950 $_{[1.450, 2.800]}$, Sync = 1.400 $_{[1.100, 2.050]}$, and OneHand = 2.000 $_{[1.500, 2.750]}$.
The temporal demand dimension results for each technique are: Simple-Ray = 3.600 $_{[2.850, 4.250]}$, Simple-Stripe = 3.250 $_{[2.600, 3.850]}$, Precision = 3.050 $_{[2.300, 3.850]}$, Sync = 3.150 $_{[2.550, 3.750]}$, and OneHand = 3.300 $_{[2.600, 3.950]}$.
The performance dimension results for each technique are: Simple-Ray = 4.300 $_{[3.400, 4.950]}$, Simple-Stripe = 4.750 $_{[3.900, 5.300]}$, Precision = 5.400 $_{[4.700, 5.900]}$, Sync = 5.200 $_{[4.450, 5.700]}$, and OneHand = 4.750 $_{[3.950, 5.300]}$.
The effort dimension results for each technique are: Simple-Ray = 3.300 $_{[2.550, 4.050]}$, Simple-Stripe = 3.550 $_{[2.750, 4.300]}$, Precision = 2.800 $_{[2.150, 3.600]}$, Sync = 2.700 $_{[1.950, 3.500]}$, and OneHand = 3.750 $_{[2.950, 4.400]}$.
The frustration level dimension results for each technique are: Simple-Ray = 2.850 $_{[2.050, 3.750]}$, Simple-Stripe = 2.800 $_{[2.100, 3.650]}$, Precision = 1.650 $_{[1.250, 2.250]}$, Sync = 1.900 $_{[1.400, 2.700]}$, and OneHand = 2.600 $_{[1.850, 3.500]}$.

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.45\textwidth]{figures/diff_plot_withB_TLX.pdf}
\caption{
Task 1 - NASA TLX comparison result. 
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:TLX_withB}   
\end{figure}

The comparison results between each technique are illustrated in Fig \ref{figure:TLX_withB}.
According to the comparison results, the Simple-Ray technique is evaluated as it requires more temporal demand (0.333 $_{[0.250, 0.400]}$) and less effort (0.233 $_{[0.200, 0.250]}$) and has a worse performance (0.433 $_{[0.350, 0.500]}$) than the Simple-Stripe technique.
Also, it requires more temporal (0.500 $_{[0.400, 0.550]}$) and mental (0.733 $_{[0.650, 0.800]}$) demands and effort (0.450 $_{[0.400, 0.500]}$), has a higher frustration level (1.167 $_{[0.800, 1.500]}$), and has a worse performance (1.117 $_{[0.950, 1.300]}$) than the Precision technique.
It requires more temporal (0.417 $_{[0.300, 0.500]}$), physical (0.550 $_{[0.450, 0.650]}$), and mental (0.567 $_{[0.550, 0.600]}$) demands and effort (0.583 $_{[0.550, 0.600]}$), has a higher frustration level (0.883 $_{[0.650, 1.050]}$), and has a worse performance (0.900 $_{[0.750, 1.050]}$) than the Sync technique.
Additionally, it requires more temporal demand (0.283 $_{[0.250, 0.300]}$) and less mental demand (0.300 $_{[0.250, 0.350]}$) and effort (0.400 $_{[0.350, 0.450]}$), has a higher frustration level (0.233 $_{[0.200, 0.250]}$), and has a worse performance (0.450 $_{[0.350, 0.550]}$) than the OneHand technique.

Next, the Simple-Stripe technique is evaluated as it requires more mental demand (0.733 $_{[0.550, 0.900]}$) and effort (0.683 $_{[0.600, 0.750]}$), has a higher frustration level (1.133 $_{[0.850, 1.400]}$), and has a worse performance (0.683 $_{[0.600, 0.800]}$) than the Precision technique.
It requires more temporal (0.083 $_{[0.050, 0.100]}$), physical (0.583 $_{[0.350, 0.800]}$), and mental (0.567 $_{[0.450, 0.650]}$) demands and effort (0.817 $_{[0.800, 0.850]}$), has a higher frustration level (0.850 $_{[0.700, 0.950]}$), and has a worse performance (0.467 $_{[0.400, 0.550]}$) than the Sync technique.
Also, it requires less mental demand (0.300 $_{[0.200, 0.350]}$) and effort (0.167 $_{[0.100, 0.200]}$) and has a higher frustration level (0.200 $_{[0.150, 0.250]}$) than the OneHand technique.

The Precision technique is evaluated as it requires more physical demand (0.550 $_{[0.350, 0.750]}$) and less mental demand (0.167 $_{[0.100, 0.250]}$), requires more effort (0.133 $_{[0.100, 0.200]}$), has a lower frustration level (0.283 $_{[0.150, 0.450]}$), and has a better performance (0.217 $_{[0.200, 0.250]}$) than the Sync technique.
Also, it requires less temporal (0.217 $_{[0.100, 0.300]}$) and mental (1.033 $_{[0.900, 1.100]}$) demand and effort (0.850 $_{[0.800, 0.950]}$), has a lower frustration level (0.933 $_{[0.600, 1.250]}$), and has a better performance (0.667 $_{[0.600, 0.750]}$) than the OneHand technique.

Lastly, the Sync technique is evaluated as it requires less temporal (0.133 $_{[0.050, 0.200]}$), physical (0.567 $_{[0.400, 0.700]}$), and mental (0.567 $_{[0.400, 0.700]}$) demand and effort (0.983 $_{[0.900, 1.050]}$), has a lower frustration level (0.650 $_{[0.450, 0.800]}$), and has a better performance (0.450 $_{[0.400, 0.500]}$) than the OneHand technique.
% The participants answered that the Simple-Ray technique requires more temporal demand but requires less effort and presents less performance than the Simple-Stripe technique.
% They answered that the Simple-Ray technique requires more temporal and mental demand and effort than the Precision technique. Also, the result shows that the Simple-Ray technique makes participants feel less performance and a higher frustration level than the Precision technique.
% In the results between the Simple-Ray technique and the Sync technique, the participants feel the Simple-Ray technique requires more temporal demand, physical demand, mental demand, and effort than the Sync technique. Also, the Simple-Ray is evaluated as having a higher frustration level but less performance than the Sync technique.
% The comparison between the Simple-Ray and OneHand technique presents that the Simple-Ray requires more temporal demand and mental demand, requires more effort, and has a higher frustration level than the OneHand technique. However, it is evaluated as having better performance than the OneHand technique.
% The Simple-Stripe technique is evaluated as requiring more mental demand and more effort, having a higher frustration level, but having worse performance than the Precision technique.
% If the Simple-Stripe technique is evaluated compared with the Sync technique, it requires more effort and makes more temporal, physical, and mental demands. Also, it is evaluated as having a higher frustration level but worse performance.
% In comparing the Simple-Stripe technique and the OneHand technique, the Simple-Stripe requires less effort and makes less mental, but it has a higher frustration level than the OneHand technique.

\subsubsection{UEQ}

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.45\textwidth]{figures/UEQ_result_withB_UEQ.pdf}
\caption{
Task 1 - UEQ. 
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:UEQ_withB}   
\end{figure}

A summary of the UEQ qualitative results are illustrated in Fig \ref{figure:UEQ_withB}.
The attractiveness scale results for each technique are: Simple-Ray = 0.625 $_{[0.025, 1.092]}$, Simple-Stripe = 0.900 $_{[0.283, 1.367]}$, Precision = 1.300 $_{[0.767, 1.758]}$, Sync = 1.417 $_{[0.783, 1.858]}$, and OneHand = 0.608 $_{[-0.033, 1.158]}$.
The perspicuity scale results for each technique are: Simple-Ray = 1.913 $_{[1.462, 2.263]}$, Simple-Stripe = 2.025 $_{[1.512, 2.400]}$, Precision = 1.962 $_{[1.312, 2.337]}$, Sync = 1.712 $_{[1.012, 2.175]}$, and OneHand = 1.825 $_{[1.450, 2.163]}$.
The efficiency scale results for each technique are: Simple-Ray = 1.225 $_{[0.675, 1.625]}$, Simple-Stripe = 1.050 $_{[0.425, 1.488]}$, Precision = 1.600 $_{[1.200, 1.913]}$, Sync = 1.738 $_{[1.312, 2.075]}$, and OneHand = 0.850 $_{[0.175, 1.288]}$.
The dependability scale results for each technique are: Simple-Ray = 0.738 $_{[0.212, 1.113]}$, Simple-Stripe = 0.975 $_{[0.400, 1.438]}$, Precision = 1.288 $_{[0.925, 1.650]}$, Sync = 1.500 $_{[1.012, 1.875]}$, and OneHand = 0.775 $_{[0.287, 1.137]}$.
The stimulation scale results for each technique are: Simple-Ray = 0.562 $_{[-0.050, 1.038]}$, Simple-Stripe = 0.787 $_{[0.212, 1.262]}$, Precision = 0.912 $_{[0.212, 1.413]}$, Sync = 1.100 $_{[0.487, 1.562]}$, and OneHand = 0.425 $_{[-0.163, 0.988]}$.
The novelty scale results for each technique are: Simple-Ray = 0.438 $_{[-0.100, 0.850]}$, Simple-Stripe = 0.525 $_{[0.175, 0.838]}$, Precision = 0.950 $_{[0.412, 1.363]}$, Sync = 1.150 $_{[0.725, 1.550]}$, and OneHand = 0.588 $_{[-0.013, 1.075]}$.


\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.45\textwidth]{figures/diff_plot_withB_UEQ.pdf}
\caption{
Task 1 - UEQ comparison results.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:diff_UEQ_withB}   
\end{figure}

The comparison results between each technique are illustrated in Fig \ref{figure:diff_UEQ_withB}.
According to the comparison results, the Simple-Ray technique is evaluated as it has less attractiveness (0.269 $_{[0.258, 0.275]}$), perspicuity (0.100 $_{[0.050, 0.138]}$), dependability (0.250 $_{[0.188, 0.325]}$), and stimulation (0.237 $_{[0.225, 0.263]}$) and has more efficiency (0.188 $_{[0.138, 0.250]}$) than the Simple-Stripe technique.
Also, it has less attractiveness (0.694 $_{[0.669, 0.742]}$), efficiency (0.396 $_{[0.287, 0.525]}$), dependability (0.600 $_{[0.542, 0.713]}$), stimulation (0.329 $_{[0.263, 0.375]}$), and novelty (0.512 $_{[0.512, 0.512]}$) than the Precision technique.
It has less attractiveness (0.772 $_{[0.758, 0.792]}$), efficiency (0.533 $_{[0.450, 0.637]}$), dependability (0.775 $_{[0.762, 0.800]}$), stimulation (0.533 $_{[0.525, 0.537]}$), and novelty (0.746 $_{[0.704, 0.825]}$) and has more perspicuity (0.246 $_{[0.087, 0.450]}$) than the Sync technique.
Additionally, it has less dependability (0.046 $_{[0.025, 0.075]}$) and novelty (0.154 $_{[0.087, 0.225]}$) and has more perspicuity (0.067 $_{[0.013, 0.096]}$), efficiency (0.404 $_{[0.338, 0.500]}$), and stimulation (0.100 $_{[0.050, 0.138]}$) than the OneHand technique.

Next, the Simple-Stripe technique is evaluated as it has less attractiveness (0.425 $_{[0.394, 0.483]}$), efficiency (0.583 $_{[0.425, 0.775]}$), dependability (0.350 $_{[0.212, 0.525]}$), and novelty (0.396 $_{[0.237, 0.525]}$) and has more perspicuity (0.108 $_{[0.062, 0.200]}$) than the precision technique.
It has less attractiveness (0.503 $_{[0.492, 0.517]}$), efficiency (0.721 $_{[0.588, 0.887]}$), dependability (0.525 $_{[0.438, 0.613]}$), stimulation (0.296 $_{[0.275, 0.312]}$), and novelty (0.629 $_{[0.550, 0.713]}$) and has more perspicuity (0.346 $_{[0.225, 0.500]}$) than the Sync technique.
Also, it has more attractiveness (0.272 $_{[0.208, 0.317]}$), perspicuity (0.167 $_{[0.062, 0.237]}$), efficiency (0.217 $_{[0.200, 0.250]}$), dependability (0.204 $_{[0.113, 0.300]}$), and stimulation (0.338 $_{[0.275, 0.375]}$) than the OneHand technique.

The Precision technique is evaluated as it has less attractiveness (0.078 $_{[0.017, 0.117]}$), efficiency (0.138 $_{[0.113, 0.163]}$), dependability (0.175 $_{[0.087, 0.225]}$), stimulation (0.204 $_{[0.150, 0.275]}$), and novelty (0.233 $_{[0.192, 0.312]}$) and has more perspicuity (0.237 $_{[0.163, 0.300]}$) than the Sync technique.
Also, it has more attractiveness (0.697 $_{[0.600, 0.800]}$), efficiency (0.800 $_{[0.625, 1.025]}$), dependability (0.554 $_{[0.512, 0.637]}$), stimulation (0.429 $_{[0.375, 0.487]}$), and novelty (0.358 $_{[0.287, 0.425]}$) than the OneHand technique.

Lastly, the Sync technique is evaluated as it has more attractiveness (0.775 $_{[0.700, 0.817]}$), efficiency (0.938 $_{[0.787, 1.137]}$), dependability (0.729 $_{[0.725, 0.738]}$), stimulation (0.633 $_{[0.575, 0.675]}$), and novelty (0.592 $_{[0.475, 0.738]}$) than the OneHand technique.


==> contents/4_2_result_boots_task_2.tex <==

\subsection{Task 2: Without Reference Object}
\subsubsection{Selection Time}

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.5\textwidth]{figures/selection_time_withoutB.pdf}
\caption{
Task 2 - Selection Time: Selection time results for each technique and each distance condition.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:ST_withoutB}   
\end{figure}

A summary of the selection time results for each technique and distance conditions in Task 2 is illustrated in Fig \ref{figure:ST_withoutB}.
The mean Selection time results for each techniques are: Simple-Ray = 2.08s $_{[1.88, 2.43]}$, Simple-Stripe = 2.28s $_{[2.11, 2.64]}$, Precision = 4.10s $_{[3.74, 4.62]}$, Sync = 3.46s $_{[3.16, 3.82]}$, and OneHand = 5.05s $_{[4.71, 5.44]}$.
The results for each distance condition to the target are: 3m = 2.81s $_{[2.55, 3.13]}$, 6m = 3.36s $_{[3.09, 3.68]}$, and 9m = 4.01s $_{[3.67, 4.41]}$.

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.5\textwidth]{figures/diff_task_2_selection_time_withoutB.pdf}
\caption{
Task 2 - Selection Time Comparison: Selection time result comparisons between each technique and each distance condition.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:diff_ST_withoutB}   
\end{figure}

A summary of the selection time comparison results between technique conditions and between target distance conditions in Task 2 is illustrated in Fig \ref{figure:diff_ST_withoutB}.
The selection time result comparisons between each technique condition show that using the Simple-Ray technique is 0.150s $_{[0.028, 0.229]}$ faster than Simple-Stripe, 2.025s $_{[1.865, 2.189]}$ faster than Precision, 1.349s $_{[1.284, 1.384]}$ faster than Sync, and 2.939s $_{[2.837, 3.001]}$ faster than OneHand techniques' results.
Simple-Stripe's result is also 1.875s $_{[1.636, 2.161]}$ faster than Precision's, 1.199s $_{[1.055, 1.356]}$ faster than Sync's, and 2.788s $_{[2.609, 2.983]}$ faster than OneHand's result.
The result from the Precision technique is 0.676s $_{[0.581, 0.805]}$ slower than from the Sync technique but 0.914s $_{[0.822, 0.972]}$ faster than from the OneHand technique.
Lastly, the Sync technique's result is 1.590 $_{[1.553, 1.627]}$ faster than OneHand's result.
Between the distances to the target position condition present that the 3m condition shows 0.549s $_{[0.545, 0.551]}$ faster result than 6m, 1.201s $_{[1.152, 1.276]}$ faster result than 9m distance condition.
Also, 6m condition shows 0.653s $_{[0.605, 0.726]}$ faster result than 9m condition.


\subsubsection{Error Distance}


\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.5\textwidth]{figures/error_distance_withoutB.pdf}
\caption{
Task 2 - Error Distance: Error distance result for each technique and each distance condition.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:ED_withoutB}   
\end{figure}

A summary of the error distance results for each technique and distance conditions in Task 1 is illustrated in Fig \ref{figure:ED_withoutB}.
The mean Error distance results from each technique condition are: Simple-Ray = 84.696cm $_{[66.769, 115.311]}$, Simple-Stripe = 61.336cm $_{[50.339, 75.411]}$, Precision = 46.207cm $_{[37.853, 56.490]}$, Sync = 37.962cm $_{[31.426, 47.753]}$, and OneHand = 71.241cm $_{[62.523, 82.688]}$.
The results for each distance condition to the target are: 3m = 24.870cm $_{[21.608, 29.149]}$, 6m = 57.744cm $_{[50.697, 66.653]}$, and 9m = 98.252cm $_{[86.974, 115.159]}$.


\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.5\textwidth]{figures/diff_task_2_error_distance_withoutB.pdf}
\caption{
Task 2 - Error Distance Comparison: Error Distance result comparisons between each technique and each distance condition.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:diff_ED_withoutB}   
\end{figure}

A summary of the error distance comparison results between techniques and between target distance conditions in Task 1 is illustrated in Fig \ref{figure:diff_ED_withoutB}.
Comparisons between error distance results with using each technique are as follows: error distance by Simple-Ray technique is 26.564cm $_{[16.430, 39.900]}$ longer than by Simple-Stripe, 42.075cm $_{[28.916, 58.821]}$ longer than by Precision, 49.878cm $_{[35.343, 67.558]}$ longer than Sync, 16.775cm $_{[4.246, 32.623]}$ longer than OneHand technique.
The Simple-Stripe technique's result show 15.512cm $_{[12.485, 18.921]}$ longer than Precision and 23.315cm $_{[18.913, 27.658]}$ longer than Sync technique's result but 9.789cm $_{[7.277, 12.184]}$ smaller than OneHand technique's result.
The result from the Precision technique is 7.803cm longer than the result from the Sync technique but 25.301cm smaller than the result from the OneHand technique.
The Sync technique's result also shows a 33.104cm $_{[31.097, 34.935]}$ smaller error distance than the result from the OneHand technique.

Results between distance conditions show that when the target is at 3m, the error distance is 33.156cm smaller than at 6m and 74.919cm $_{[68.038, 86.010]}$ smaller than at 9m. Also, the result at 6m is 41.763cm $_{[37.687, 48.506]}$ smaller than at 9m.

\subsubsection{NASA TLX}

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.45\textwidth]{figures/TLX_result_withoutB_TLX.pdf}
\caption{
Task 2 - NASA TLX. 
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:TLX_withoutB}   
\end{figure}

A summary of the NASA-TLX qualitative results are illustrated in Fig \ref{figure:TLX_withoutB}.
The mental demand dimension results for each technique are: Simple-Ray = 3.150 $_{[2.400, 3.800]}$, Simple-Stripe = 2.850 $_{[2.150, 3.700]}$, Precision = 3.000 $_{[2.300, 3.750]}$, Sync = 3.100 $_{[2.300, 3.950]}$, and OneHand = 4.250 $_{[3.350, 5.000]}$.
The physical demand dimension results for each technique are: Simple-Ray = 1.850 $_{[1.400, 2.450]}$, Simple-Stripe = 1.700 $_{[1.300, 2.450]}$, Precision = 1.900 $_{[1.350, 2.750]}$, Sync = 1.650 $_{[1.300, 2.200]}$, and OneHand = 1.850 $_{[1.350, 2.450]}$.
The temporal demand dimension results for each technique are: Simple-Ray = 3.750 $_{[3.000, 4.400]}$, Simple-Stripe = 3.850 $_{[3.150, 4.500]}$, Precision = 3.600 $_{[2.900, 4.300]}$, Sync = 3.400 $_{[2.650, 4.050]}$, and OneHand = 3.850 $_{[3.150, 4.500]}$.
The performance dimension results for each technique are: Simple-Ray = 4.850 $_{[3.950, 5.450]}$, Simple-Stripe = 4.950 $_{[4.000, 5.450]}$, Precision = 5.350 $_{[4.400, 5.850]}$, Sync = 4.800 $_{[3.858, 5.300]}$, and OneHand = 3.650 $_{[2.950, 4.200]}$.
The effort dimension results for each technique are: Simple-Ray = 3.250 $_{[2.400, 4.000]}$, Simple-Stripe = 2.800 $_{[2.250, 3.400]}$, Precision = 3.250 $_{[2.450, 4.000]}$, Sync = 2.750 $_{[2.050, 3.500]}$, and OneHand = 4.000 $_{[3.100, 4.700]}$.
The frulstration level dimension results for each technique are: Simple-Ray = 2.350 $_{[1.750, 3.050]}$, Simple-Stripe = 1.950 $_{[1.450, 2.700]}$, Precision = 1.950 $_{[1.450, 2.600]}$, Sync = 1.950 $_{[1.450, 2.742]}$, and OneHand = 2.850 $_{[2.100, 3.750]}$.

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.45\textwidth]{figures/diff_plot_withoutB_TLX.pdf}
\caption{
Task 2 - NASA TLX comparison result. 
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:TLX_withoutB}   
\end{figure}

The comparison results between each technique are illustrated in Fig \ref{figure:TLX_withoutB}.
According to the comparison results, the Simple-Ray technique is evaluated as it requires less temporal demand (0.117 $_{[0.100, 0.150]}$) and more mental demand (0.217 $_{[0.100, 0.300]}$) and effort (0.400 $_{[0.150, 0.600]}$) and has a higher frustration level (0.350 $_{[0.300, 0.400]}$) than the Simple-Stripe technique.
Also, it requires more temporal (0.117 $_{[0.100, 0.150]}$) and mental (0.100 $_{[0.050, 0.150]}$) demands, has a higher frustration level (0.383 $_{[0.300, 0.450]}$), and has a worse performance (0.450 $_{[0.400, 0.500]}$) than the Precision technique.
It requires more physical demand (0.183 $_{[0.100, 0.250]}$) and effort (0.450 $_{[0.350, 0.500]}$), has a higher frustration level (0.336 $_{[0.300, 0.400]}$), and has a better performance (0.097 $_{[0.050, 0.150]}$) than the Sync technique.
Additionally, it requires less temporal (0.117 $_{[0.100, 0.150]}$) and mental (1.083 $_{[0.950, 1.200]}$) demands and effort (0.717 $_{[0.700, 0.750]}$), has a lower frustration level (0.517 $_{[0.350, 0.700]}$), and a better performance (1.150 $_{[1.000, 1.250]}$) than the OneHand technique.

Next, the Simple-Stripe technique is evaluated as it requires more temporal demand (0.233 $_{[0.200, 0.250]}$) and less physical (0.183 $_{[0.050, 0.300]}$) and mental (0.117 $_{[0.050, 0.150]}$) demands and effort (0.417 $_{[0.200, 0.600]}$) and has a better performance (0.400 $_{[0.400, 0.400]}$) than the Precision technique.
It requires more temporal demand (0.467 $_{[0.450, 0.500]}$) and less mental demand (0.217 $_{[0.150, 0.250]}$) and has a better performance (0.147 $_{[0.141, 0.150]}$) than the Sync technique.
Also, it requires less mental demand (1.300 $_{[1.200, 1.400]}$) and effort (1.117 $_{[0.850, 1.300]}$), has a lower frustration level (0.867 $_{[0.650, 1.050]}$), and has a better performance (1.200 $_{[1.050, 1.300]}$) than the OneHand technique.

The Precision technique is evaluated as it requires more temporal (0.233 $_{[0.200, 0.250]}$) and physical (0.283 $_{[0.050, 0.550]}$) demands and effort (0.467 $_{[0.400, 0.500]}$) and has a better performance (0.547 $_{[0.541, 0.550]}$) than the Sync technique.
Also, it requires less temporal (0.233 $_{[0.200, 0.250]}$) and mental (1.183 $_{[1.050, 1.250]}$) demands and effort (0.700 $_{[0.650, 0.750]}$), has a lower frustration level (0.900 $_{[0.650, 1.150]}$), and has a better performance (1.600 $_{[1.450, 1.700]}$) than the OneHand technique.

Lastly, the Sync technique is evaluated as it requires less temporal (0.467 $_{[0.450, 0.500]}$), physical (0.167 $_{[0.050, 0.250]}$), and mental (1.083 $_{[1.050, 1.150]}$) demand and effort (1.167 $_{[1.050, 1.250]}$), has a lower frustration level (0.853 $_{[0.650, 1.008]}$), and has a better performance (1.053 $_{[0.908, 1.150]}$) than the Onehand technique.

\subsubsection{UEQ}

\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.45\textwidth]{figures/UEQ_result_withoutB_UEQ.pdf}
\caption{
Task 2 - UEQ. 
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:UEQ_withoutB}   
\end{figure}

A summary of the UEQ qualitative results are illustrated in Fig \ref{figure:UEQ_withoutB}.
The attractiveness scale results for each technique are: Simple-Ray = 1.175 $_{[0.608, 1.583]}$, Simple-Stripe = 1.142 $_{[0.358, 1.692]}$, Precision = 1.583 $_{[1.067, 2.017]}$, Sync = 1.308 $_{[0.667, 1.717]}$, and OneHand = 0.183 $_{[-0.508, 0.833]}$.
The perspicuity scale results for each technique are: Simple-Ray = 2.312 $_{[1.800, 2.575]}$, Simple-Stripe = 2.038 $_{[1.325, 2.462]}$, Precision = 2.112 $_{[1.538, 2.462]}$, Sync = 2.000 $_{[1.312, 2.425]}$, and OneHand = 1.100 $_{[0.525, 1.650]}$
The efficiency scale results for each technique are: Simple-Ray = 1.587 $_{[1.200, 1.900]}$, Simple-Stripe = 1.575 $_{[1.000, 1.975]}$, Precision = 1.750 $_{[1.350, 2.075]}$, Sync = 1.812 $_{[1.250, 2.125]}$, and OneHand = 0.787 $_{[0.212, 1.287]}$
The dependability scale results for each technique are: Simple-Ray = 1.087 $_{[0.613, 1.438]}$, Simple-Stripe = 1.238 $_{[0.787, 1.550]}$, Precision = 1.387 $_{[1.012, 1.725]}$, Sync = 1.325 $_{[0.825, 1.675]}$, and OneHand = 0.375 $_{[-0.225, 0.825]}$
The stimulation scale results for each technique are: Simple-Ray = 0.863 $_{[0.250, 1.312]}$, Simple-Stripe = 0.875 $_{[0.138, 1.413]}$, Precision = 1.212 $_{[0.650, 1.663]}$, Sync = 1.200 $_{[0.650, 1.538]}$, and OneHand = 0.225 $_{[-0.396, 0.750]}$
The novelty scale results for each technique are: Simple-Ray = 0.775 $_{[0.275, 1.175]}$, Simple-Stripe = 0.800 $_{[0.362, 1.238]}$, Precision = 1.200 $_{[0.762, 1.550]}$, Sync = 1.100 $_{[0.700, 1.475]}$, and OneHand = 0.725 $_{[0.000, 1.212]}$


\begin{figure}[t]
\centering
\includegraphics[angle=0, width=.45\textwidth]{figures/diff_plot_withoutB_UEQ.pdf}
\caption{
Task 2 - UEQ comparison results.
% VR Experiment: Detection Rate Results (95\% CI error bar)
} 
\label{figure:diff_UEQ_withoutB}   
\end{figure}

The comparison results between each technique are illustrated in Fig \ref{figure:diff_UEQ_withoutB}.
According to the comparison results, the Simple-Ray technique is evaluated as it has less dependability (0.146 $_{[0.113, 0.175]}$) and novelty (0.058 $_{[0.025, 0.087]}$) and has more perspicuity (0.287 $_{[0.113, 0.475]}$) than the Simple-Stripe technique.
Also, it has less attractiveness (0.433 $_{[0.408, 0.458]}$), efficiency (0.163 $_{[0.150, 0.175]}$), dependability (0.329 $_{[0.292, 0.400]}$), stimulation (0.367 $_{[0.350, 0.400]}$), and novelty (0.429 $_{[0.375, 0.487]}$) and more perspicuity (0.192 $_{[0.113, 0.263]}$) than the Precision technique.
It has less attractiveness (0.108 $_{[0.058, 0.133]}$), efficiency (0.167 $_{[0.050, 0.225]}$), dependability (0.229 $_{[0.212, 0.237]}$), stimulation (0.321 $_{[0.225, 0.400]}$), and novelty (0.350 $_{[0.300, 0.425]}$) and more perspicuity (0.317 $_{[0.150, 0.487]}$) than the Sync technique.
Additionally, it has more attractiveness (0.953 $_{[0.750, 1.117]}$), perspicuity (1.137 $_{[0.925, 1.275]}$), efficiency (0.800 $_{[0.613, 0.988]}$), dependability (0.721 $_{[0.613, 0.838]}$), and stimulation (0.615 $_{[0.562, 0.646]}$) than the OneHand technique.

Next, the Simple-Stripe technique is evaluated as it has less attractiveness (0.492 $_{[0.325, 0.708]}$), dependability (0.183 $_{[0.150, 0.225]}$), efficiency (0.208 $_{[0.100, 0.350]}$), stimulation (0.367 $_{[0.250, 0.512]}$), and novelty (0.371 $_{[0.400, 0.312]}$) than the precision technique.
It has less attractiveness (0.167 $_{[0.025, 0.308]}$), efficiency (0.212 $_{[0.150, 0.250]}$), dependability (0.083 $_{[0.037, 0.125]}$), stimulation (0.321 $_{[0.125, 0.512]}$), and novelty (0.292 $_{[0.237, 0.338]}$) and more perspicuity (0.029 $_{[0.013, 0.037]}$) than the Sync technique.
Also, it has more attractiveness (0.894 $_{[0.858, 0.958]}$), perspicuity (0.850 $_{[0.800, 0.938]}$), efficiency (0.754 $_{[0.688, 0.787]}$), dependability (0.867 $_{[0.725, 1.012]}$), stimulation (0.615 $_{[0.534, 0.658]}$), and novelty (0.154 $_{[0.025, 0.362]}$) than the OneHand technique.

The Precision technique is evaluated as it has more attractiveness (0.325 $_{[0.275, 0.400]}$), perspicuity (0.125 $_{[0.037, 0.225]}$), dependability (0.100 $_{[0.050, 0.188]}$), and novelty (0.079 $_{[0.062, 0.100]}$) than the Sync technique.
Also, it has more attractiveness (1.386 $_{[1.183, 1.575]}$), perspicuity (0.946 $_{[0.812, 1.012]}$), efficiency (0.963 $_{[0.788, 1.137]}$), dependability (1.050 $_{[0.900, 1.238]}$), stimulation (0.982 $_{[0.912, 1.046]}$), and novelty (0.525 $_{[0.338, 0.762]}$) than the OneHand technique.

Lastly, the Sync technique is evaluated as it has more attractiveness (1.061 $_{[0.883, 1.175]}$), perspicuity (0.821 $_{[0.775, 0.900]}$), efficiency (0.967 $_{[0.838, 1.038]}$), dependability (0.950 $_{[0.850, 1.050]}$), stimulation (0.936 $_{[0.787, 1.046]}$), and novelty (0.446 $_{[0.263, 0.700]}$) than the OneHand technique.

==> contents/5_discussion.tex <==
\section{Discussion}

In this section, we discuss our findings from the study on mid-air selection, its limitations, and our future research directions.

\paragraph{Simple-Ray} % Simple-Ray
% (두 Task 모두에서 Simple-Ray technique은 Simple-Stripe을 제외한 다른 supporting feature가 있는 bimanual 기술들과 OneHand technique과 비교해 가장 빠른 선택을 사용자에게 제공하였다. 이는 Simple-Stripe을 제외한 다른 technique들과 비교해서 가장 조작이 직관적이고 간단하기 때문에 그렇다 볼 수 있다.
% 그러나 흥미롭게도 참가자들의 workload 설문 결과, Simple-Ray technique은 Task 1에서 Temporal demand가 가장 높은 것으로 조사되었다.
% 반면 Task 2에서는 그러지 않았다.
% 이 차이점으로부터 Simple-Ray technique은 limited range 안을 선택할 때, 사용자에게 Temporal pressure를 가한다고 짐작 할 수 있다.
% 이는 다른 technique과 달리 supporting feature가 없기 때문에 가능한 빠르게 limited range 내를 선택해야 하는 task 1에서는 temporal demand가 크게 느껴지기 때문일 것이다.
% 또한 기억에 의존하여 원하는 위치를 선택하는 task 2에서는 마찬가지로 가능한 빠르게 선택을 해야 하지만 느껴지는 temporal damand가 significant 하게 크진 않기 때문일 것이다.

% Simple-Ray technique은 Task 1에서는 Precision을 제외한 다른 technique에 비해 정확했지만 participants는 Simple-Ray가 가장 낮은 performance를 가진다고 평가했다.
% 또한 dependability가 다른 모든 techniques에 비해 낮게 평가되었는데, 이로써 task 1과 같은 정밀한 선택을 해야하는 환경에서 Simple-Ray technique은 다른 bimanual techniques에 비해 실제 결과에 상관없이 사용자는 secure 하다고 느끼지 못함을 알 수 있다.

% Task 2에서 Simple-Ray technique은 가장 부정확하였고 사용자들은 Simple-Ray technique이 다른 bimanual technique에 비해 다른 scales은 모자라지만 perspicuity 하다고 응답하였다.
% 이는 어떤 supporting feature도 없이 가장 간단한 technique임에 나온 평가로 보인다.
% 사용자들은 OneHand보다는 정확했다고 느꼈고, Novelty를 제외한 모든 UEQ scale에서 OneHand보다 낫다는 평가를 하였다.
% 즉, 원하는 Mid-air position을 선택할 때, bimanual technique이 unimanual technique 보다 사용자에게 더 나은 경험을 선사 할 수 있다는 것을 보여준다.
% )
In both tasks, the Simple-Ray technique offers the participants the fastest selection compared to other selection techniques except the Simple-Stripe technique.
This can be attributed to its comparatively more intuitive and straightforwardness than other techniques, requiring additional control using a joystick.
However, interestingly, the participants answer the workload survey (NASA-TLX) that the Simple-Ray technique has the highest temporal demand in Task 1.
We can guess that this perception difference is due to the participants having the pressure to select the target position accurately within a limited range as quickly as possible without any supporting features\cite{angrilli1997influence}.
In contrast, the temporal demand is not significantly high in task 2, which asks the participants to select where they remember.

In task 1, the Simple-Ray technique is the most accurate one except for the Precision technique, but the participants answer they felt it has the worst performance.
Moreover, in the UEQ result, the Simple-Ray technique's dependability is evaluated worse than all other techniques. Thus, we can guess that, when a user has to select a mid-air position accurately, such as in task 1, the user can not trust the Simple-Ray technique independent of the actual result.

In task 2, the Simple-Ray technique is the most inaccurate compared to all other techniques.
This can be guessed as because there is no support feature to help with depth perception or control sensitivity.
However, the participants answer the Simple-Ray technique has a better performance, stimulation, perspicuity, efficiency, dependability, and attractiveness than the OneHand technique.
Consequently, we can consider that even the basic bimanual selection technique can provide a better experience to a user than the unimanual technique when selecting a mid-air position where the user wants to select.

% In both tasks, the Simple-Ray technique allows the participants to select the target position faster than other bimanual techniques with supporting features and the OneHand technique.
% However, interestingly, according to the participants' workload questionnaire results for this technique in task 1, the temporal demand is at the highest level compared to other techniques.
% In contrast, the Simple-Ray technique's temporal demand in task 2 is not the highest.
% From this difference, we can guess that the Simple-Ray technique exercises temporal pressure on a user when making an accurate selection into a limited range.
% Moreover, although the selection accuracy in task 1 is better than that of other techniques except the Precision technique, the accuracy in task 2 is the worst.
% From that, even though the Simple-Ray does not have any supporting features, 


% Fastest selection % Task 1
% Fastest selection % Task 2

% Less accuracy than Precision, better accuracy than others % Task 1
% Less accuracy than all others % Task 2

% The highest Temporal demand / The least performance % Task 1 - TLX
% Less stimulation than other bimanual techniques, less dependability than all other techniques, better efficiency than OneHand% Task 1 - UEQ
% Become less temporal demand than Simple-Stripe and OneHand. Better performance than OneHand.% Task 2 - TLX
% Task 2 - UEQ

\paragraph{Simple-Stripe} % Simple-Stripe
% (Simple-Stripe technique은 Simple-Ray technique과 마찬가지로 두 Task 모두에서 참가자들이 다른 selection techniques를 사용하였을 때 보다 빠르게 target position을 선택 할 수 있게 하였다.

% Task 1에서 Simple-Stripe technique은 사용자들이 OneHand technique 보다는 정확한 선택을 할 수 있도록 하였지만 흥미롭게도 Simple-Ray technique을 이용한 선택보다는 inaccurate 한 결과를 보여주었다. 심지어 참가자들도 Simple-Stripe technique이 Simple-Ray technique보다 inefficiency 하다는 응답을 하였다. 또한 Simple-Stripe이 더 많은 effort를 요구한다고 응답하였는데, Simple-Stripe과 Simple-Ray technique의 차이가 dominant hand에 있는 1m 길이의 줄무늬뿐인걸 고려하면 이 줄무늬를 고려해 target position을 선택하려 할때 더 많은 effort가 필요하고 그로인해 Simple-Stripe이 Simple-Ray에 비해 inefficiency 하고 inaccurate 한 결과를 가져왔다고 짐작 할 수 있다.
% 즉, task 1과 같은 정밀한 선택을 해야하는 상황에선 depth perception을 증가시켜 줄 것이라 예상되었던 stripes이 오히려 정확한 선택을 방해하고 사용자의 경험을 안좋게 한다 할 수 있다.

% Task 2에서 Simple-Stripe은 Precision이나 Sync와 같은 accurate selection을 support 해주는 feature를 가진 bimanual technique을 제외한 다른 모든 경우보다 accurate한 결과를 가져왔다. 이는 Simple-Stripe에 있는 줄무늬가 Mid-air position의 위치를 기억하고 선택하는데 도움을 주었지만 여전히 정밀한 선택을 하는데는 추가적인 feature가 필요하다고 볼 수 있다.
% 하지만 참가자들은 다른 bimanual techniques와 비교해서 Simple-Stripe이 더 높은 temporal demand를 요구한다고 응답 하였는데, 실제 다른 technique을 이용해서 target position을 선택하는데 걸린 시간은 Simple-Stripe technique을 이용할때와 같거나 (Simple-Ray) 긴것을 고려하면 사용자들이 Sripe을 이용해 depth perception을 할때 temporal pressure를 느낄 가능성이 있다.
% 즉, task 2처럼 Mid-air position을 기억 / 선택 해야 하는 경우에 Stripe이 도움이 될 수 있으나 이를 이용할때 사용자 경험이 감소 할 수 있을 수 있다.)
Like the Simple-Ray technique, the Simple-Stripe technique offers the participants the fastest selection compared to other techniques.
The reason is also guessed to be the same as simple and intuitive control.
In task 1, with the Simple-Stripe technique, participants can select the mid-air position more accurately than the OneHand technique.
However, interestingly, even though this technique has supporting features, the result is more inaccurate than the result from the Simple-Ray technique.
Furthermore, the answers from the participants indicate that they felt the Simple-Stripe technique was more inefficient than the Simple-Ray technique.
Also, they answer that more effort is needed to use the Simple-Stripe than the Simple-Ray.
Due to the only difference between the Simple-Stripe and the Simple-Ray is 1m length stripes, we can guess that having an accurate selection within the limited range using the stripes makes a user have to put in more effort.
That can be a reason for the inaccurate selection and participants feeling inefficient.
Consequently, the stripes, which we expected to increase the depth perception, can disrupt the accurate selection and decrease the quality of the user experience in situations like task 1.

In task 2, the Simple-Stripe technique led to a more accurate selection result than the Simple-Ray and OneHand techniques.
However, the accuracy is worse than the results with the Precision or Sync technique, which has a supporting feature for helping selection.
The comparison between results from the Simple-Stripe and Simple-Ray techniques makes us guess that the stripes help a user remember where a target position was. Also, we can guess that a support feature to help with an accurate selection can increase the selection accuracy of the Simple-Stripe technique.
The participants feel the Simple-Stripe technique has more temporal demand than all other bimanual techniques. However, the actual selection time results show that the Simple-Stripe is one of the fastest selection techniques in task 2. Thus, a user may feel temporal pressure when using the stripes feature in task 2, such as using the Simple-Ray technique case.
Consequently, in a mid-air selection situation such as task 2, the Stripes can help increase the selection accuracy, but it can decrease the user experience.
% Fastest selection % Task 1
% Fastest selection % Task 2

% Less accuracy than Simple-Ray and Precision / No difference with Sync / better accuracy than OneHand % Task 1
% Less accuract than Precision and Sync / better accuracy than all others % Task 2

% The highest effort compared with other bimanual techniques. The higher frustration level than others except the Simple-Ray. % Task 1 - TLX
% Best perspicuity. Better than OneHand for all scales % Task 1 - UEQ

% More temporal demand than all other bimanual techniques. Better performance than OneHand.% Task 2 - TLX
% Task 2 - UEQ

\paragraph{Precision-Stripe} % Precision
% (Precision technique을 이용한 경우 두 Task 모두에서 참가자들이 다른 bimanual techniques를 사용하였을 때 보다 느리게 target position을 선택 할 수 있었지만 OneHand technique을 사용하였을 때 보다는 빠른 선택이 가능하다. 이는 range selection을 하기 위해 controller의 joystick을 조절하는 시간이 필요하기 때문으로 보인다.
% Task 1에서 Precision technique은 가장 정확한 selection 결과를 만들었으며 사용자들도 최고의 performance를 가지는 technique으로 느꼈다 응답하였다. 게다가 mental demand와 frustration level이 다른 technique과 비교해 가장 낮음을 고려하면 선택 가능한 range를 제한하는 것이 사용자가 limited range 안의 위치를 정확하게 선택하는데 도움을 주고 사용자의 부담을 덜어준다 할 수 있다.
% 하지만 사용자들은 UEQ 설문지에서 Precision technique이 OneHand와 Simple-Ray를 모든 scale에서 더 좋다 응답했으나 Simple-Stripe보다는 perspicuity가 낮다고 응답하였다. 이는 Limited Range 안의 지정된 위치를 선택해야 하는 task 1에서는 selected range가 지정된 위치를 포함하고 있는지 확인하고 그안에서 다시 정확한 target position을 선택해야 하기 때문에 나온 결과로 보인다. 후술하겠지만 Sync technique에서도 동일한 결과를 얻을 수 있었다.
% 즉, task 1과 같은 상황에선 range selection feature가 performance에는 긍정적인 영향을 가져오지만 perspicuity와 같은 user experience에는 긍정적이지 않다.

% Task 2에서 Precision technique은 참가자들이 Sync technique을 제외한 다른 technique 보다 정확한 selection을 할 수 있게 만들었다. Target position을 기억하는 단계에선 Simple-Stripe과 차이가 없다는 점을 고려하면 이는 range selection feature가 사용자가 선택하려는 위치를 정확하게 선택할 수 있도록 도와주었다 볼 수 있다.
% 참가자들은 Precision이 다른 모든 techniques보다 나은 performance를 보인다고 응답하였다.
% 하지만 Simple-Stripe technique에 비해 높은 physical, mental demand와 effort를 가지고 있다고 응답하였다. Precision technique과 Simple-Stripe technique의 차이점을 고려하면, 가까이에 위치한 target position을 선택하는 경우에도 불필요하게 controller의 joystick을 움직여 range selection supporing feature를 사용해야만 하기 때문일 것으로 보인다.
% )
With the Precision technique, participants can select the target position faster than with the OneHand technique but slower than with other bimanual techniques.
We can guess that the reason is that the Precision technique needs extra time to move the selected range using a joystick.

In task 1, the Precision technique produces the most accurate selection result, and participants' workload survey results show this technique's performance as the best.
Moreover, mental demand and frustration level are surveyed as the lowest compared with other techniques. As a result, we can consider that range selection support helps a user to select the target position accurately and decreases the user burden in a situation like task 1.
However, the UEQ results show that the Precision technique is better than the OneHand and Simple-Ray techniques for all scales. However, perspicuity is less than the Simple-Stripe.
We guess that is because the Precision technique should select a range to limit the position of the crossing point.
When a user selects a position where the user wants, such as task 2, the selecting range is not an issue.
However, when a user has to select a designated position accurately within a range limit, such as task 1, there is an additional step to check the chosen range is within the range limit.
We guess that is the reason why the Precision technique has less perspicuity in task 1. Similary, the Sync technique also has less perspicuity than the Simple-Stripe in task 1.

In task 2, the Precision technique produces the most accurate selection result except the Sync technique. Considering this technique is not different from the Simple-Stripe technique at the position remember step for each trial, the selection range feature to limit the position of the crossing point can be thought to help the accurate selection.
The NASA-TLX results present this Precision technique has a better performance than all other techniques, but the UEQ results show this technique has more physical and metal demand and requires more effort than the Simple-Stripe.
If comparing these two techniques, these higher demands and efforts come from the additional step for selecting a range. Also, it can be because the Precision technique should select a range even if the position a user wants to select is close enough to choose without any support.
% Faster than OneHand / Slower than all others % Task 1
% Faster than OneHand / Slower than all others % Task 2

% The most accuracy than all others % Task 1
% Less accuracy than Sync / better accuracy than Simple-Ray, Simple-Strip, OneHand% Task 2

% The least mental demand. The best performance. The lowest frustration level. + all dimenstions are better than OneHand. % Task 1 - TLX
% Better than OneHand and Simple-Ray for all scales, Better than Simple-Stripe except perspicuity% Task 1 - UEQ
% Better performance than all other techniques.% Task 2 - TLX
% Task 2 - UEQ

\paragraph{Cursor-Sync} % Sync
% (
% Sync technique을 이용한 경우 두 task 모두에서 참가자들은 Simple-Ray와 Simple-Stripe techniques를 이용했을 떄 보다는 target position 선택이 느렸지만 Precision과 OneHand technique을 사용한 경우 보다는 빠르게 선택할 수 있다. 이는 Simple-Ray와 Simple-Stripe보다는  range를 선택하는데 시간이 걸리지만, Sync feature를 통한 향상된 controllability 를 통해 selected range안에서 원하는 위치를 빠르게 선택 할 수 있었던 것으로 보인다.

% Task 1에선 참가자들은 Sync technique을 사용해 OneHand보단 정확한 선택을 하였지만 Simple-Ray와 Precision techniques들에 비해선 부정확한 선택을 하였고 Simple-Stripe과 비슷한 정도의 정확도를 보여주었다. 이는 Precision technique의 결과와 비교하였을 때 Sync feature가 task 1의 환경에선 accuracy에 도움을 주지 못하고 심지어 range selection feature을 통해 향상된 정확도를 상쇠할 정도로 부정적인 영향을 끼쳤다.

% 하지만 사용자들은 Sync technique의 Physical demand가 다른 모든 techniques보다 낮다고 응답했다. 이는 멀리 위치한 target position을 선택 할 때 sync feature가 향상시킨 controllability로 인한 결과로 보인다. 또한 UEQ 결과, 사용자들은 Sync technique이 OneHand보다는 모든 scale에서 낫고, 다른 bimanual technique보다는 perspicuity를 제외한 나머지 scale에서 낫다고 응답하였다. 이는 first stripe에서 crossing point를 조작하는 것이 직관적이지 않은 탓으로 보인다.

% Task 2에서 Sync technique은 다른 모든 techniques과 비교해 가장 정확한 결과를 가져왔으며 이는 sync feature가 selected range 내에서 정확한 선택을 할 수 있도록 controllabilty를 향상시킨 결과라 볼 수 있다. 게다가 참가자들은 Sync technique이 Precision보다 더 적은 Mental과 physical demand와 effort를 요구한다 응답하였는데, 이는 sync feature가 사용자들이 Precision technique에서 겪던 가장 큰 문제인 control sensitivity를 해결해 주었기 때문으로 보인다.
% )
With the Sync technique condition, participants select the target position faster than the Precision and OneHand techniques.
We guess that the Sync feature increases controllability compared to the Precision technique and makes for rapid selection.
Also, the selection is slower than the Simple-Ray and Simple-Stripe techniques, and it may be because the Sycn technique needs more time to select a range limit.

In task 1, the error distance results show that the Sync technique is more accurate than the OneHand technique but less accurate than the Simple-Ray and Precision techniques.
If compared with a result from the Precision technique, the Sync feature, which controls a crossing point in the first stripe, does not increase selection accuracy and even decreases accuracy.

However, in the NASA-TLX result, participants answer the physical demand of the Sync technique is the lowest compared with all other techniques. We guess it is because the sync feature can make it easy to control the far away crossing point within the first stripe.
Also, in the UEQ result, participants answer the Sync technique is better than all other techniques for all evaluation scales except perspicuity when compared with other bimanual techniques.
We guess that is because the sync feature, control the remote crossing point, is not intuitive.

In task 2, the Sync technique is the most accurate technique in this study. We guess it is because the Sync technique helps control a far-away crossing point within a close region. Also, the participants feel the Sync technique has fewer mental and physical demands and requires less effort than the Precision technique.

We suppose that it is because the sync feature solves a control sensitivity issue when selects a far-away position in the Precision technique.

% Faster than OneHand, Precision / Slower than others % Task 1
% Faster than OneHand, Precision / Slower than others % Task 2

% Less accuracy than Simple-Ray and Precision / No difference with Simple-Stripe / better accuracy than OneHand % Task 1
% The best accuracy than all others% Task 2

% The lowest physical demand + all dimenstions are better than OneHand.% Task 1 - TLX
% (Worse performance than Precision)
% Better than OneHand for all scales. Better than Simple-Ray, Simple-Stripe, and precision except perspicuity% Task 1 - UEQ
% Less Mental, Physical demands and Effort than Precision. Better performance than OneHand.% Task 2 - TLX
% Task 2 - UEQ

% \paragraph{A high frustration level technique makes a user feel they need to spend more time.}
% Task 2: OneHand = Highest frustration level + Highest Temporal demand -> Highest selection time.
% But
% Task 1: Simple-Ray (Highest frustration level + Highest Temporal demand) -> Lowest selection time.

% %Distance
% When the target is located closer, the selection time and error distance are decreased in both tasks.
% However, it is not clear whether this difference in accuracy results from better depth perception or better selection control at a close distance.

% -------------------------------------------------------------------

% Task 1:
% The Simple-Ray and Simple-Stripe show the fastest selection, but users felt that have the highest frustration level.
% (The simplest controlling, but users felt selecting the position with these techniques is frustrating.)
% However, the Simple-Stripe technique's error distance result shows that this technique has less accuracy than the Simple-Ray technique.
% (Stripe may be disrupting the depth perception?)
% The Precision technique is slower than the Sync technique.
% (The Sync process decrease the time for handling the cross point.)
% The OneHand technique is the slowest technique in this task.
% (It shows bimanual technique can have a rapid selection.)

% The Simple-Ray technique's error distance result is smaller than the OneHand technique and larger than the Precision technique.
% (It because the Simple-Ray does not have a supporting feature for accurate selection. It shows that even though there is no supporting feature, bimanual mid-air selection is more accurate than the unimanual technique.)
% However, the Sync technique does not present a better accuracy (less error distance) than the Simple-Ray technique, even it has additional features.
% (This result indicate that the direct aiming of the target position is more important than the accurate control.)

% Even though the Simple-Ray technique provides the fastest selection, the participants feel this technique has the highest temporal demand compared to others.
% (Why?)
% Also, they feel that the OneHand technique has the highest mental demand and effort.
% ()
% The performance evaluation of the participants presents the Precision technique has the best performance.
% (This indicates that the direct aiming of the target position with the range selection makes the participants feel that it is working well.)

% The participants evaluate the Simple-Ray technique as the least novelty, dependability, and attractiveness but the highest perspicuity.
% (Hard to select the position, but easy to learn and use it)
% However, the Sync technique is evaluated as having the least perspicuity but the highest stimulation, novelty, efficiency, dependability, and attractiveness.
% (The Sync technique makes participants feel good to use but also feel the most complex.)


% Task 2:

% The Simple-Ray and Simple-Stripe show the fastest selection.
% ()


% The Sync technique is the most accurate technique.
% ()
% The Simple-Ray is the most inaccurate and the OneHand is the next.
% ()

% Participants evaluate the One-Hand technique as it requires the highest temporal, physical, and mental demands and effort. They also feel the One-Hand technique makes them highly frustrated (highest frustration level) and its performance is the worst.
% ()
% Also, they feel the Sync technique requires the least temporal, physical demand and effort and has the lowest frustration level.
% ()
% However, the selection time result presents the Simple-Ray and Simple-Stripe as the fastest techniques.
% ()


% (TLX):
% Temporal Demand: Sync / OneHand
% Physical Demand: Sync, Simple-Stripe / Simple-Ray, Precision, OneHand
% Performance: OneHand / Precision
% Mental Demand: Simple-Stripe / OneHand
% Frustration Level: Simple-Stripe, Precision, Sync / OneHand
% Effort: Simple-Stripe, Sync / OneHand

% In task 2, participants evaluate the OneHand technique as the worst for all scales in UEQ, stimulation, perspicuity, novelty, efficiency, dependability, and attractiveness compared with all other techniques.
% Except for perspicuity, the Precision technique is evaluated as the highest scale for all scales. The technique with the highest perspicuity is Simple-Ray.

% (UEQ):
% Stimulation: OneHand / Precision
% Perspicuity: OneHand / Simple-Ray
% Novelty: Simple-Ray, OneHand / Precision
% Efficiency: OneHand / Precision, Sync
% Dependability: OneHand / Precision
% Attractiveness: OneHand / Precision


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

